Compressed Factorization: Fast and Accurate Low-Rank Factorization of Compressively-Sensed Data

What learning algorithms can be run directly on compressively-sensed data? In this work, we consider the question of accurately and efficiently computing low-rank matrix or tensor factorizations given data compressed via random projections. We examine the approach of first performing factorization in the compressed domain, and then reconstructing the original high-dimensional factors from the recovered (compressed) factors. In both the matrix and tensor settings, we establish conditions under which this natural approach will provably recover the original factors. While it is well-known that random projections preserve a number of geometric properties of a dataset, our work can be viewed as showing that they can also preserve certain solutions of non-convex, NP-Hard problems like non-negative matrix factorization. We support these theoretical results with experiments on synthetic data and demonstrate the practical applicability of compressed factorization on real-world gene expression and EEG time series datasets.

==> expander.tex <==
\section{Proof of expander property: Lemma \ref{expander}}\label{sec:expander}

In this section, we provide a proof of our claim that randomly chosen projection matrix is an expander with the desired expansion. This is Part 2 of Lemma \ref{expander}. Part 1 is used in the proof of uniqueness for NMF (Lemma \ref{lem:exp1}).

\expander*
\begin{proof}
	Consider any subset $S\subset U$ with $|S|\le \gamma n_1$. Let $\Prob(N(S)\subseteq M)$ denote the probability of the event that the neighborhood of $S$ is entirely contained in $M\subset V$. $\Prob(N(S)\subseteq M) \le \Big(\frac{|M|}{n_2}\Big)^{D|S|}$. We will upper bound the probability of $G$ not being an expander by upper-bounding the probability of each subset $S\subset U$ with $|S|\le \gamma n_1$ not expanding. Let $\Prob(\bar{S})$ denote the probability of the neighborhood of $S$ being entirely contained in a subset $M\subset V$ with $M< {\alpha} |S|D$. By a union bound,
	\begin{align}
	\Prob(G \text{ is not a $(\gamma n_1,\alpha)$ expander}) &\le \sum_{\substack{S\subset U\\ |S|\le \gamma n_1}}^{} \Prob(\bar{S})\nonumber\\
	&\le \sum_{\substack{S\subset U\\ |S|\le \gamma n_1}}^{} \sum_{\substack{M\subset V\\ M= {\alpha} |S|D}}^{}\Prob(N(S)\subseteq M)\nonumber\\
	&\le  \sum_{s=1}^{\gamma n_1}\sum_{\substack{S\subset U\\ |S|= s}}^{} \sum_{\substack{M\subset V\\ M= {\alpha} |S|D}}^{} \Big(\frac{{\alpha} |S|D}{n_2}\Big)^{D|S|}\nonumber\\
	&\le   \sum_{s=1}^{\gamma n_1} {n_1 \choose  s}{n_2 \choose {\alpha} Ds}\Big(\frac{{\alpha} Ds}{n_2}\Big)^{Ds}\nonumber\\
	&\le   \sum_{s=1}^{\gamma n_1} \Big(\frac{n_1 e}{  s}\Big)^{{\alpha} s}\Big(\frac{n_2 e}{ {\alpha} Ds}\Big)^{{\alpha} Ds}\Big(\frac{{\alpha} Ds}{n_2}\Big)^{Ds}\nonumber\\
	&\le \sum_{s=1}^{\gamma n_1} \Bigg[ \Big(\frac{n_1 e}{  s}\Big)^{{\alpha} }\Big(\frac{n_2 e}{ {\alpha} Ds}\Big)^{{\alpha} D}\Big(\frac{{\alpha} Ds}{n_2}\Big)^{D} \Bigg]^s\nonumber\\
	&\le \sum_{s=1}^{\gamma n_1} x_s^s\nonumber
	\end{align}
	where $x_s= \Big(\frac{n_1 e}{  s}\Big)^{ }\Big(\frac{n_2 e}{ {\alpha} Ds}\Big)^{{\alpha} D}\Big(\frac{{\alpha} Ds}{n_2}\Big)^{D} $. $x_s$ can be bounded as follows-
	\begin{align}
	x_s &= \Big(\frac{n_1 e}{  s}\Big)\Big( \frac{{\alpha} D s e^{1/{(1-\alpha)}}}{n_2} \Big)^{{(1-\alpha)} D}\nonumber\\
	&\le \Big(\frac{e}{ \gamma }\Big)\Big( \frac{{\alpha} D \gamma n_1 e^{1/(1-\alpha)}}{n_2} \Big)^{{(1-\alpha)} D}\nonumber\\
	&\le \Big(\frac{n_1 e^{1+1/(1-\alpha)}}{n_2}\Big)D{\alpha}^{{(1-\alpha)}D }\nonumber\\
	&\le \Big(\frac{n_1 e^{6}}{n_2}\Big)De^{-D/25}
	= x\nonumber
	\end{align}
	where in the last step we set $\alpha=4/5$. Hence we can upper bound the probability of $G$ not being an expander as follows---
	\begin{align}
		\Prob(G \text{ is not a $(\gamma n_1,\alpha)$ expander}) \le \sum_{s=1}^{\infty}x^s \le  \frac{x}{1-x}\nonumber
	\end{align}
	The two parts of Lemma \ref{expander} follow by plugging in the respective values for $n_1, n_2$ and $D$.
\begin{comment}
	We now bound $x$ separately to prove the two parts of Lemma \ref{expander}.
	\begin{enumerate}
		\item For $n_1=n^c$ and $n_2 = n$, we bound $x$ as follows,
		\begin{align}
		x &=  \Big(\frac{n_1 e^{2}}{n_2}\Big)De^{-0.3D}\nonumber\\
		&\le \frac{e^2}{n^{1-c}}ke^{-0.3k} \nonumber
		\end{align}
		\item For $n_1>n_2$, we bound $x$ as follows,
		\begin{align}
		x &=  \Big(\frac{n_1 e^{2}}{n_2}\Big)re^{-0.3r}\nonumber\\
		&\le \Big(\frac{n_2}{n_1}\Big)\nonumber
		\end{align}
		for $r=10\log(n_1/n_2)$.
		
	\end{enumerate}
\end{comment}	
\end{proof}

==> experiments-old.tex <==
\section{Empirical Evaluation}
\label{sec:experiments}

The goal of this section is the following:

1. Compare \textsc{Factorize-Recover} with  \textsc{Recover-Factorize} in terms of runtime and reconstruction error for matrix and tensor factorizations on real-world domains where compressed sensing has been applied. %(gene expression levels and EEG). 
We focus most of our matrix factorization evaluation on NMF.\\
2. Provide empirical evidence that sparsity of the underlying factors is the key requirement for \textsc{Factorize-Recover} to succeed by computing a dense factorization, SVD, with \textsc{Factorize-Recover} and through synthetic experiments where the sparsity of the factors can be controlled.

We defer additional synthetic experiments which show that most of the error \textsc{Factorize-Recover} incurs happens mostly in the recovery step and not in the factorization step, and additional evaluation of the EEG factors for the detection of seizures to the Appendix.

% 1) compare the \textsc{Factorize-Recover} with the \textsc{Recover-Factorize} approach in terms of runtime and reconstruction error for matrix and tensor factorizations on real-world domains where compressed sensing has been applied (gene expression levels and EEG); 2) 

%In this section, we evaluate the empirical performance of NMF and TD on compressed data.We focus on two domains where compressed measurement and data transmission have been applied: measurements of gene expression levels and EEG time series. In addition to real-world datasets for evaluating the practical applicability of these methods, we also perform a sensitivity analysis on synthetic data for which true low-rank factorizations are known.

When evaluating on real-world data, we simulate compressive measurements by projecting the data with sparse random binary matrices $P\in\{0,1\}^{d\times n}$ where each column has 5 nonzero entries.\footnote{We presents an analysis of the trade-off between the sparsity of $P$ and reconstruction accuracy in the Appendix.}

%\paragraph{Measurement Matrices.}
%Recall that Theorem~\ref{thm:nmf} guarantees a correspondence between sparse solutions in the original and compressed space when the projection matrix $P$ corresponds to the adjacency matrix of a bipartite expander graph. 
%In our experiments, we use projection Count-Min sketch \citep{cormode2005improved}

\subsection{Non-Negative Matrix Factorization}

\paragraph{Gene Expression Data.} %Gene expression measurements play an important role in the biological sciences: for instance, they can be used to predict clinical outcomes for individuals with certain forms of cancer \citep{pomeroy2002prediction,mills2009microarray}. NMF has been  widely-used tool for unsupervised learning of gene expression data due to the interpretability of the discovered factors \citep{gao2005improving,kim2007sparse}. 
NMF has been  widely-used tool for unsupervised learning of gene expression data \citep{gao2005improving,kim2007sparse}. Since the dictionary factors obtained by NMF on gene expression data have been empirically observed to be sparse, this domain is well-suited for testing our proposed NMF approach. 

A DNA microarray is a device used to measure the expression levels of thousands of genes simultaneously. The underlying gene expression levels are sparse and hence  \emph{compressed microarrays} \citep{parvaresh2008recovering,dai2008compressive,cleary2017efficient} incorporate ideas from compressive sampling into DNA microarray design by measuring the expression levels of combinations of genes in each slot. Due to practical design limitations, the measurement matrices for compressed microarrays are both \emph{sparse} and \emph{non-negative}. We evaluated our proposed NMF approach on gene expression datasets targeting three disease classes: embryonal central nervous system tumors \citep{pomeroy2002prediction}, lung carcinomas \citep{bhattacharjee2001classification}, and leukemia \citep{mills2009microarray}. These datasets are summarized in Table~\ref{table:gene-timing}. Each dataset is represented as a real-valued matrix where the $i$th row denotes expression levels for the $i$th gene across each sample.

\begin{table*}

  \caption{Summary of DNA microarray gene expression datasets, along with runtime (seconds) for each stage of NMF pipeline on compressed data. \textsc{Factorize-Recover} runs only $r$ instances of sparse recovery, as opposed to the (\# samples) instances used by \textsc{Recover-Factorize}.}
  \label{table:gene-timing}
  \centering
  \begin{tabular}{@{}rccrrcrr@{}}
  \toprule
  \multirow{2}{*}{Dataset} &
\multirow{2}{*}{\# Samples} &
\multirow{2}{*}{\# Features} &
   \multicolumn{2}{c}{\textsc{Recover-Fac.}} & \phantom{a} & \multicolumn{2}{c}{\textsc{Fac.-Recover}} \\
   \cmidrule(l){4-5} \cmidrule(l){7-8}
     & &     & Recovery & NMF && NMF & Recovery \\
  \midrule
  CNS tumors & 266 & 7,129 & 76.1 & 2.7 && 0.6 & 5.4 \\
  Lung carcinomas & 203 & 12,600 & 78.8 & 4.0 && 0.8 & 9.3 \\
  Leukemia & 435 & 54,675 & 878.4 & 39.6 && 6.9 & 55.0 \\
  \bottomrule
  \end{tabular}
 % \vspace{4pt}
\end{table*}

\vspace{-10pt}
\paragraph{Experimental Setup.} For all datasets, we fixed a rank of $r=10$; this choice is consistent with previous clustering analyses in this domain \citep{gao2005improving,kim2007sparse}. 
For each data matrix $X\in\mathbb{R}^{n\times m}$, we simulated compressed measurements $\tilde{M}\in\mathbb{R}^{d \times m}$ by projecting the feature dimension: $\tilde{M} = PX$.
%The measurement matrix $\tilde{M}$ was used as input to the \textsc{Recover-Factorize} and \textsc{Factorize-Recover} procedures.
We performed NMF by running projected gradient descent \citep{lin2007projected} for 250 iterations---this was sufficient to reach convergence on our datasets.
 
\vspace{-10pt}
\paragraph{Computation Time.} Computation time for NMF on all 3 datasets  (Table~\ref{table:gene-timing}) is dominated by the cost of solving instances of the $\ell_1$-minimization problem (\ref{eq:basis-pursuit}). %\footnote{We measured runtimes on a machine with a 2.5GHz Intel i7 CPU with 4 cores and 16GB RAM. We solved the LP problems using the SCS solver \citep{scs}.} 
As a result, \textsc{Factorize-Recover} achieves much lower runtime as it requires a factor of $m / r$ fewer calls to the sparse recovery procedure. %Note that the recovery times do not exactly scale by this factor, possibly due to differences in problem conditioning.

\vspace{-10pt}
\paragraph{Reconstruction Error vs. Compression.}  We compared the reconstruction error in the Frobenius norm achieved by \textsc{Recover-Factorize} versus \textsc{Factorize-Recover} at varying compression levels, $n/d$.
The error was computed relative to the original data $X$.
 Figure~\ref{fig:gene-plot} summarizes our results. 
We found that for a fixed number of measurements, NMF in the compressed domain achieved better reconstruction error than in the uncompressed domain at compression factors above $3\times$, with a decrease in error of up to $30\%$ on the Leukemia dataset. 
We observed a similar accuracy gap when testing variants of the factorization and recovery procedures: in particular, when performing sparse recovery using the Lasso instead of LP-based recovery, and when regularizing NMF with an $\ell_1$ penalty on $W$.
The existence of such a substantial accuracy gap is perhaps surprising---we investigate this phenomenon further in our experiments on synthetic data.

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{figs/nmf-gene.pdf}
	\caption{Normalized Frobenius errors $\|X-WH\|_F / \|X\|_F$ for NMF on gene expression data with varying compression factors $n/d$. \textbf{Solid:} \textsc{Factorize-Recover}. \textbf{Dotted:} \textsc{Recover-Factorize}. \textbf{Dashed:} error on original, uncompressed data with error bars. Above $\sim3\times$ compression, NMF on compressed data achieves lower reconstruction error than NMF after sparse recovery.}
	\label{fig:gene-plot}
\end{figure*}

\vspace{-4pt}

\subsection{Empirical analysis of conditions under which \textsc{Factorize-Recover} works}

\paragraph{SVD with \textsc{Factorize-Recover}.} Does \textsc{Factorize-Recover} outperform \textsc{Recover-Factorize} for other matrix factorization methods? Figure~\ref{fig:nmf-svd} shows that the improvement seen for NMF does not hold for SVD on the CNS dataset: FR-SVD results in higher error than RF-SVD. This discrepancy is due to the fact that the SVD factorization is less sparse than the NMF factorization.\footnote{This is reflected in empirical measures of sparsity: the mean Gini index \citep{hurley2009comparing} over the columns of the left factor for SVD was 0.70, while for NMF it was 0.84. The Gini index is continuous value in $[0, 1]$, where values closer to 1 indicate sparser vectors.} This result indicates that sparsity is crucial for the success of \textsc{Factorize-Recover}.

\begin{figure}
  \centering
  \includegraphics[width=3 in]{figs/nmf-svd.pdf}
  \caption{FR-NMF outperforms RF-NMF on the CNS dataset, but the opposite is true for SVD. Sparse factorizations are necessary for \textsc{Factorize-Recover} to work well.}
  \label{fig:nmf-svd}
\end{figure}

%\vspace{-10pt}


%\vspace{-6pt}
%\paragraph{Projection Sparsity.}

%\begin{figure}
%  \includegraphics[width=\columnwidth]{figs/nmf-sparsity.pdf}
%  \caption{Normalized Frobenius errors for NMF on lung carcinoma dataset vs. column sparsity of projection $P$.}
%  \label{fig:nmf-sparsity}
%\end{figure}

%\vspace{-6pt}
%\paragraph{Alternatives to LP-based Recovery.} SSMP

\vspace{-10pt}
\paragraph{Synthetic Experiments.} To explore the observed gap in reconstruction accuracy between the \textsc{Recover-Factorize} and \textsc{Factorize-Recover} procedures for NMF, we perform experiments on synthetic data. We generate approximately low-rank data $X = WH + \varepsilon$, where $W = B\odot G$ for random binary $B$ with column sparsity $k$, each entry of $G$ is the absolute value of an i.i.d. $N(0,1)$ variable, each $H_i$ is sampled from $\mathrm{Dirichlet}(\alpha)$ for a given $\alpha > 0$, and the noise term $\varepsilon$ is a random Gaussian matrix. The Dirichlet distribution allows us to control the sparsity of $H$. We form the measurement matrix as usual: $\tilde{M} = PX$. In Figure~\ref{fig:nmf-synthetic}, we show the effect of varying the rank of $WH$ and the sparsity of $H$ (via $\alpha$) while holding fixed the factor sparsity $k$ and the signal-to-noise ratio of the data. As the rank increases or the sparsity of $H$ decreases, the sparsity of each sample (i.e., column of $X$) decreases. This harms per-sample sparse recovery since more measurements are required for accurate recovery. FR-NMF is more robust to these changes than RF-NMF since the factor $PW$ is sparser than the individual samples, and therefore is more amenable to sparse recovery. Thus, NMF benefits from representing each sample as a mixture of sparse basis vectors (effectively ``sparsifying'' the inputs to the sparse recovery procedure).

\begin{figure}
	\centering
  \includegraphics[width=3 in]{figs/nmf-synthetic.pdf}
  \caption{Comparing FR-NMF with RF-NMF on synthetic data. We varied the rank of $WH$ and the sparsity of $H$ (measured by the Gini index) at fixed $n=5000$, $m=100$, $k = 0.01n$, and $\mathrm{SNR} = 0.1$. The FR procedure is more robust due to the sparsity of the factors obtained by NMF.}
  \label{fig:nmf-synthetic}
\end{figure}

\subsection{Tensor Decomposition}

\paragraph{Compressed EEG Time Series.} %Scalp EEG measurements are used to monitor electrical activity in the brain over time. 
Scalp EEG readings are typically organized as a collection of time series (``channels''), where each series corresponds to a measurement of electrical activity in a different region of the brain. Order-3 tensors can be derived from this data by computing short-time Fourier transforms (STFTs) for each channel: this yields a tensor where each slice is a time-frequency matrix. Tensor decomposition can then be applied to cluster patterns of neural activity that are common across time and across different channels \citep{cong2015tensor}. In the EEG setting, random projections are used as a computationally cheap data compression technique. This approach is particularly useful for portable monitoring devices in order to reduce storage requirements and bandwidth usage in data transmission \citep{abdulghani2012compressive,zhang2013compressed,craven2015compressed}.

The CHB-MIT Scalp EEG Database \citep{shoeb2010application} is a collection of scalp EEG recordings of children susceptible to epileptic seizures.
We computed per-channel STFTs for EEG recordings from one patient in the dataset (\texttt{CHB01}) to obtain a tensor of size
$27804\times303\times23$ ($\mathrm{time} \times \mathrm{frequency} \times \mathrm{channel}$), corresponding to approximately 40 hours of data.
%We expect that this data should exhibit the desired sparsity property since EEG signals typically exhibit well-localized time-frequency structure.
We computed a rank-10 non-negative decomposition of this tensor using projected CP-ALS \citep{kolda2009tensor}, and 
we compressed the data by projecting along the first (temporal) axis using a sparse binary matrix with column sparsity 5.

\vspace{-2pt}
{\vspace{.45em}\noindent\textbf{Results.}} In Figure~\ref{fig:td}, we show normalized Frobenius errors of the recovered factorization and median Pearson correlations between the columns of the recovered temporal factor and those computed on the original, uncompressed data (paired via maximum bipartite matching). Due to the sparsity of the data, we can achieve over $10\times$ compression at the cost of a $14\%$ increase in reconstruction error. RF-TD achieves slightly lower error at a given projection dimension: at $d=1000$, RF-TD achieves a normalized error of $0.819$ vs. $0.834$ for FR-TD. However, RF-TD is three orders of magnitude slower than FR-TD on this dataset due to the large number of sparse recovery instances required ($303\times 23 = 6969$) to fully recover the data tensor.

\begin{figure}
  \centering
  \includegraphics[width=3 in]{figs/td.pdf}
  \caption{FR-TD on compressed EEG data. \textbf{Left:} Normalized Frobenius error; dashed line indicates baseline reconstruction error on original data. \textbf{Right:} Median Pearson correlations between recovered factors and factors computed from original data.}
  \label{fig:td}
\end{figure}

%\paragraph{Synthetic Data.}



==> fig1.tex <==
\begin{tikzpicture}[shorten >=1pt,>=stealth',thick]

%\draw (0, 1) -- (2, 1) -- (2, 3) -- (0, 3) -- (0, 1);
%\draw ()
\node (Mtilde) at (0, 1.1) {$\tilde{M}$};
\node (Mtilde_label) at (0, 0.4) {\begin{tabular}{c}compressed\\data\end{tabular}};
\node (M) at (5, 1.1) {$M$};
\node (M_label) at (5, 0.4) {\begin{tabular}{c} recovered\\sparse data \end{tabular}};

\node (WHtilde) at (0, -1.1) {$\tilde{W}, \tilde{H}$};
\node (WHtilde_label) at (0, -1.8) {\begin{tabular}{c} compressed \\ factorization \end{tabular}};
\node (WH) at (5, -1.1) {$W, H$};
\node (WH_label) at (5, -1.8) {\begin{tabular}{c} recovered sparse \\ factorization \end{tabular}};

%\node (A1) at (0.4, -0.55)  {$A_1$};

\draw [->,black!50!green] (Mtilde_label) to node[left]{factorize} (WHtilde);
\draw [->,black!20!red] (M_label) to node[right]{factorize} (WH);
\draw [->,black!50!green] (WHtilde_label.north east) to node[below]{recover} (WH_label.north west);
\draw [->,black!20!red] (Mtilde_label.north east) to node[below]{recover} (M_label.north west);

% \begin{tabular}{c} sparse \\ recovery \end{tabular}

%\node (xy) at (0, 1.05) {$(\mathbf{x}_t, y_t)$};
%\node (nabla) at (1.75, 1.05) {$\nabla \hat{L}_t$};
%\node (gridtop) at (3.5, 1.25) {};
%\node (gridbot) at (3.5, 0.8) {};
%\node (gridright) at (4.65, 1.06) {};
%\node (feats) at (6.25, 1.1) {\begin{tabular}{@{}rr@{}} \small{``foo''} & \small{2.5}  \\ \small{``bar''} & \small{-1.9} \\ \small{``baz''} & \small{1.8} \end{tabular}};
%
%\draw [step=0.2, shift={(3.5, 0.8)}] (0, 0) grid (1.2, 0.6);
%
%\node (data) at (0, -0.12) {\begin{tabular}{c} streaming \\ data \end{tabular}};
%\node (grad) at (1.75, -0.12) {\begin{tabular}{c}  gradient \\ estimates \end{tabular}};
%\node (z) at (4.1, -0.12) {\begin{tabular}{c} sketched \\ classifier \end{tabular}};
%\node (approx) at (6.25, -0.12) {\begin{tabular}{c}estimates of \\ largest weights \end{tabular}};
%
%\draw [->] (xy) -- (nabla);
%\draw [->] (nabla) to [bend left=30] node[above]{\small update} (gridtop);
%\draw [->] (gridbot) to [bend left=30] node[below]{\small query} (nabla);
%\draw [->] (gridright) to (feats);

%\node [draw, inner sep=2mm] (f) at (0, 0) {$\phi$};
%\node (tall) at (-2, 1) {$v$(tall)};
%\node (tree) at (-2,-1) {$v$(tree)};
%\node (talltree) at (2.5, 0) {$v$(tall tree)};

%\draw [->] (tall) -- (f);
%\draw [->] (tree) -- (f);
%\draw [->] (f) -- (talltree);
\end{tikzpicture}

==> introduction_icml.tex <==
\section{Introduction}

% compressive sensing
Compressive sensing is a method for acquiring sparse signals using far fewer measurements than the ambient dimension of the data \citep{donoho2006compressed}. %In particular, any $k$-sparse vector $x \in \mathbb{R}^n$ can be exactly recovered using only $d = O(k\log(n/k))$ linear measurements of the data \citep{donoho2006compressed}. 
Since many real-world signals are indeed sparse in some basis (e.g., the Fourier basis), compressive sensing has found widespread application in a variety of domains \citep{qaisar2013compressive}. The use of compressive measurement has enabled higher throughput in signal acquisition, more compact sensors, and reduced data storage cost \citep{duarte2008single,candes2008introduction}.

In many applications where compressed sensing is used, the end goal is not to just recover the original signal, but to subsequently learn a machine learning model for a downstream task. A natural question to ask then is if it is possible to directly learn the machine learning model from the compressed data. This would not only help further understand compressed sensing theoretically, but could also yield significant computational benefits by avoiding the expensive sparse recovery step on every data sample. In light of these implications, there has been significant interest in understanding what operations can be directly performed on compressed data for tasks some of which are learning linear classifiers \citep{calderbank2009compressed,durrant2010compressed}, PCA \citep{fowler2009compressive,zhou2011godec,ha2015robust}, regression \citep{zhou2009compressed,maillard2009compressed,kaban2014new} and signal processing \citep{shoaib2015signal}.  

% low rank factorizations / setting
The goal of this work is to understand settings under which low-rank matrix and tensor factorizations can be directly performed on compressed data. Low-rank matrix and tensor factorizations are well-established tools for unsupervised learning on high-dimensional data \cite{berry2007algorithms,kolda2009tensor}, and are widely used in domains where data is acquired via compressive measurement. For example, non-negative matrix factorization (NMF) of gene expression data has been used to cluster tissue samples corresponding to different forms of cancer \citep{gao2005improving}, while tensor decomposition (TD) has been used to analyze EEG data in order to identify distinct modes of brain activity \cite{cong2015tensor}. In both these domains, compressive sensing techniques have been applied as a means of efficient data acquisition \citep{parvaresh2008recovering} and bandwidth-limited data transmission \citep{zhang2013compressed}.

% problem
The canonical approach to computing these factorizations with compressively-sensed data is to first perform sparse recovery on each sample, then run a low-rank factorization algorithm on the recovered matrix or tensor. We refer to this approach as the \textsc{Recover-Factorize} (RF) procedure: first perform sparse recovery on each sample, then run a low-rank factorization algorithm on the recovered matrix or tensor.
The problem with this approach is that sparse recovery of a full dataset typically involves solving a linear program for each sample \citep{candes2006near,donoho2006compressed}, and the cost of this step can be a computational bottleneck for large datasets.

\begin{figure}
  \centering
%  \includegraphics[width=3 in]{fig1}
  \input{fig1}
  \caption{Two possible approaches to computing low-rank factorization of compressively-sensed data: factorizing recovered data (\textsc{\color{black!20!red}Recover-Factorize}) or factorizing compressed data directly (\textsc{\color{black!50!green}Factorize-Recover}). In this work, we show that the latter confers substantial runtime and accuracy benefits when the projected factors are sparse.}
\end{figure}

% proposal
%Instead of performing low-rank factorization on the recovered data, a natural idea is to reverse the order of operations: first perform factorization on the compressed data, and then run sparse recovery to obtain the factors in the original space. 
In this paper, we analyze an alternative approach---\textsc{Factorize-Recover} (FR)---in which the order of operations is reversed: we first factorize the compressed data, then perform sparse recovery to obtain factors in the original space. Pushing down the factorization step can have significant computational benefits---instead of running (\# samples)-instances of sparse recovery, this strategy only incurs a cost proportional to the target rank, which is typically small (on the order of 10-50, compared to 1000s of samples). In practice, performing factorization directly on compressed data can improve runtime by several orders of magnitude.

However, it is not clear that \textsc{Factorize-Recover} should work well in theory or in practice.
Consider the following motivating example for NMF. 
The data $M\in\mathbb{R}^{n \times m}$ is generated as a product of nonnegative matrices: $M = WH$, $W\in\mathbb{R}^{n\times r}$ and $H \in \mathbb{R}^{r \times m}$, where $W$ is sparse. 
We observe the compressed measurements $\tilde{M}=PM$ for a known measurement matrix $P\in\mathbb{R}^{d\times n}$. 
If NMF on $\tilde{M}$ obtains the factorization $\tilde{M} = (PW)H$, then sparse recovery on each column of $PW$ will successfully recover the true factor $W$. 
%However, though low-dimensional projections can preserve geometric properties such as pairwise distances \cite{kane2014sparser}, it is not  clear that they should preserve solutions to non-convex, NP-Hard \cite{vavasis2009complexity} problems such as NMF.
Although $\tilde{M} = (PW)H$ is one possible solution to the NMF problem on $\tilde{M}$, this factorization is in general not unique; thus, it appears possible for NMF to return a ``bad'' solution that, after performing sparse recovery, is a poor approximation to the original matrix $M$.
We therefore ask: does there exist some distinguishing property of the ``good'' solution $\tilde{M} = (PW)H$ that allows us to recover it in practice?

%However, the NMF problem is NP-hard \citep{arora2012computing} and non-convex with multiple local minima \cite{vavasis2009complexity}. Therefore, we can ask: does there exist some distinguishing property of the solution $\tilde{M} = (PW)H$ such that we should expect to recover it in practice?

% but at the price of solving a convex program in order to recover the original, high-dimensional data.

%Matrix and tensor factorization are widely-used tools for the unsupervised discovery of structure in data. However, a significant difficulty with these methods that is often encountered in practice is that computing factorizations for high-dimensional matrices and tensors can be computationally expensive. For example, non-negative matrix factorization typically involves computing iterates on a sequence of constrained least-squares problems, which is computationally expensive in high dimension.
%matrix factorization with constraints on the factors---\emph{e.g.}, non-negative matrix factorization---typically involves computing iterates on a sequence of constrained least-squares problems. 

% proposal
%In this work, we propose a method that leverages a structural assumption on the factors of the matrix or tensor that we wish to decompose in order to accelerate the computation of the factorization. In particular, we assume that at least one of the factor matrices in the decomposition is \emph{sparse}. This sparsity structure is frequently seen in practice, for example in matrices and tensors derived from textual data \citep{CITE}, medical imaging \citep{CITE}, and spectral analyses of time series \citep{CITE}.
%Importantly, we note that even though the underlying factors of interest are sparse, the data itself may be dense due to contamination by dense noise.

% what are the difficulties here?
%Our method is the following: (1) we project the data to lower dimension using an appropriately-chosen random projection, (2) we run the matrix or tensor factorization algorithm on this compressed version of the original data, and (3) we recover the factorization in the original dimensionality using a sparse recovery algorithm. 
%This approach is a natural combination of two popular tools: random projections for dimensionality reduction, and compressive sensing for approximate recovery of data from a small number of measurements.
%However, it is not clear that these methods should work well in combination for computing matrix or tensor factorizations.
%First, in order for the sparse recovery step to be successful, we require that the low-dimensional factor be a linear projection of the high-dimensional factor, and it is not clear that this should be true.
%Second, the projection and sparse recovery steps both need to be sufficiently fast in order to realize computational gains in practice.
%This approach draws on now-classic techniques from compressive sensing, where high-dimensional data can be approximately recovered from a small number of random measurements of the data. 

\vspace{-12pt}

\paragraph{Our contributions.} In this work, we answer the above question in the affirmative.
We show the following theoretical guarantee for sparse matrix factorization: if the original left-factor $W$ is sparse in each column, then the projection $PW$ is the sparsest possible left-factor for a non-negative factorization of the compressed data.
This result provides theoretical grounding for why we should expect \textsc{Factorize-Recover} with sparse matrix factorization methods to succeed in practice.
In particular, we focus on low-rank matrix factorization with NMF---it has been empirically observed that NMF often learns sparse dictionaries on real-world data~\citep{lee1999learning}, and it is also common practice to use $\ell_1$-regularization on the factors to explicitly encourage sparse solutions~\citep{hoyer2004non}.
Moreover, we provide empirical evidence that sparsity is the key determinant of success for \textsc{Factorize-Recover} by demonstrating that its application to SVD---which typically returns denser factorizations than NMF---fails to recover accurate low-rank approximations. 
In addition to our main theoretical contribution on sparse matrix factorization, we also show theoretically that \textsc{Factorize-Recover} works for tensor decomposition.

We empirically validate our approach by performing NMF on several real-world gene expression datasets targeting a range of diseases---a domain where compressive sensing has emerged as a promising approach for high-throughput data acquisition~\citep{parvaresh2008recovering,dai2008compressive,cleary2017efficient}. We also evaluate TD on compressed EEG data derived from children susceptible to epileptic seizures. We find that performing factorization on compressed data achieves reconstruction accuracy comparable to or better than factorization on recovered data. Perhaps surprisingly, in many NMF instances, the factorizations obtained on the compressed data outperformed those obtained on the recovered data---for example, on one gene expression dataset, we observe up to 30\% improvement in Frobenius reconstruction error. We hypothesize that this phenomenon is due to the sparsifying effect of the NMF procedure, and support this claim with empirical evidence.

%We develop a simple framework for computing sparse factorizations and investigate it in the context of non-negative matrix factorization (NMF) and tensor
%decomposition. We show that our approach recovers the true solution with a negligible error across several synthetic and real datasets. Empirically, sparse learning allows $5\times$ compression with negligible loss in accuracy on real data, and obtains up to $2\times$ speedups in terms of wall clock time to obtain the same accuracy.

%Theoretically establishing \emph{why} such speed-ups and high fidelity reconstructions are possible and justified requires care: we establish novel uniqueness guarantees for NMF which demonstrate that if the original factors are sparse, then the projection of the factors of the original, high-dimensional NMF problem is the \emph{sparsest} possible factorization for the low-dimensional projected NMF problem. As NMF algorithms implicitly~\cite{lee1999learning} or explicitly~\cite{hoyer2004non} learn sparse factorizations, our results explain why the factorization is preserved by projection, explaining the empirical success of our procedure. Our results do not assume separability~\cite{donoho2004does} of the NMF factors, a commonly used---but very strong---assumption for showing uniqueness of NMF. We also derive simple conditions for uniqueness and provable recovery for tensor decomposition in the projected space. These theoretical insights, backed by our empirical findings, illustrate the benefits of random projections to compute sparse factorizations.



%In what settings can sparse factorization be learned more efficiently than their dense analogs?  Sparse models commonly arise in feature selection
%(e.g., diagnostic
%tasks~\cite{tibshirani1996regression, guyon2003introduction,kim2013root,
% bailis2017macrobase}), in problems with few, highly indicative
%features (e.g., time-series
%prediction~\cite{bai2008forecasting,huang2010predicting}), and in
%resource-constrained environments (i.e., a sparse model is needed for
%more efficient inference~\cite{fowers,hanfpga}).  In these tasks, sparsity can reduce the data requirements for a desired predictive power, and improve interpretability and inference speed; and a range of popular techniques provide means of learning
%these sparse models from dense and/or high-dimensional
%data~\cite{sparsitybook1,sparsitybook2}. In this work, we study an
%additional dimension of sparse models: the extent to which a model’s sparsity can be leveraged for a \emph{computational} advantage.
%
%We present a general and efficient approach to learning sparse factorizations
%that explicitly leverages the target model sparsity. We adapt now-classic
%techniques from compressive sensing~\cite{candes2006near,berinde2008combining} in a simple framework for learning
%sparse models from high-dimensional data: (1) project data to a
%lower-dimensional subspace using a random projection, (2) learn a dense factorization in this
%lower-dimensional subspace, then (3) recover a sparse factorization in the
%original dimensionality using compressive sensing. This approach has several benefits. First, it allows us to perform the bulk of model training in an often much lower-dimensional dense subspace, offering in significant efficiency gains when data is high-dimensional and the target model is sparse. Second, it is useful in settings where the dataset is very large and cannot be fit in memory; our approach allows us to work with a much smaller, low dimensional projection but still recover the original model. Third, it provides a conceptually simple approach to learning sparse models, combining powerful ideas from dimensionality reduction and compressive sensing.
%
%Although low-dimensional projections are extremely popular tools for speeding up a variety of optimization and learning problems~\cite{woodruff,randnla,randmat}, our framework is conceptually different, as we are interested in being able to recover the sparse solution in the original space from the (possibly dense) solution in the lower-dimensional space, whereas most of the current literature on compressed learning focuses on projecting the data and subsequently working in the lower dimensional space itself, instead of recovering the original factors from the projected factors. Note that this is not even information theoretically possible for many tasks even if the original model or solution is sparse: if the solution in the lower-dimensional space is not a projection of the original solution, then performing a compressive sensing based recovery has no hope of recovering the original solution (even if the original solution is sparse).




%Our results on the uniqueness of NMF after random projection---and our empirical findings---open a new perspective on the properties of random projections. It is well known that random projections can preserve distances and other geometric properties (e.g.,~\cite{kane2014sparser}), but our results show that random projections can also preserve the solutions to non-convex optimization problems such as NMF. Our approach successfully leverages this property to efficiently learn sparse models, and we believe this aproach has several promising applications beyond our target settings.

% We crucially used this property to define our framework for learning sparse models, and beleive 

%We briefly outline the two main classes of sparse models we consider in this paper:

%, and defend the uniqueness and recovery of linear classifiers by drawing a link to recent results for low-rank models

%\vspace{-10pt}
%\paragraph{Non-negative Matrix Factorization (NMF).} The goal of NMF is to approximate a non-negative matrix ${M} \in \mathbb{R}^{m\times n}$ with a product of two non-negative matrices ${W} \in \mathbb{R}^{m\times r}$ and ${H} \in \mathbb{R}^{r \times n}$. The matrix $W$ is regarded as the dictionary, and $H$ stores the combination weights of each column of $M$ in terms of the dictionary $W$. Applications of NMF include document clustering~\cite{xu2003document} and image analysis~\cite{lee1999learning,li2001learning}. A crucial property of NMF that enables it to learn good representation of the data is that the coefficients $H$ are typically sparse~\cite{lee1999learning,hoyer2004non}, so that each document or image is expressed as a combination of few basis vectors in the dictionary. In settings such as document clustering or image classification, the columns of $M$ correspond to samples from the dataset (e.g., documents or images). In many scenarios, $n\gg m$, as the number of samples is large for big datasets. We are interested in this setting, where $n$ is very large but the factor $H$ is sparse.
%%\vspace{-10pt}
%\paragraph{Tensor Decomposition.} The goal of tensor decomposition is to decompose a tensor $T\in \mathbb{R}^{m_1\times m_2\times n}$ with rank $r$ in terms of its factors $T=\sum_{i=1}^{r}A_i\otimes B_i \otimes C_i$. This is the most commonly used model of tensor decomposition, and is also known as CANDECOMP/PARAFAC or CP
%decomposition. Here, $A_i$ denotes the $i$th column of the factor $A\in \mathbb{R}^{m_1\times r}$ and $\otimes$ denotes the outer product: $a,b,c\in \mathbb{R}^n$ then $a\otimes b \otimes c \in \mathbb{R}^{n\times n \times n}$ and $(a\otimes b\otimes b)_{ijk}=a_ib_jc_k$. As in NMF, we consider settings where the third mode corresponding to the factor $C$ represents data points and is very large---but sparse. The first two modes could correspond to features for each data point; for example in a topic modeling setup \cite{anandkumar2014tensor}, the first two modes could represent word co-occurrences, with the third mode representing different documents.

%\vspace{-10pt}
%Let $T(:,:,i)\in \mathbb{R}^{n_1\times n_2}$ represent the $i$th matrix slice of the tensor
% for vectors $a,b,c$ $(a\otimes b\otimes b)_{ijk}=a_ib_jc_k$
% $a,b,c\in \mathbb{R}^n$ then $a\otimes b \otimes c \in \mathbb{R}^{n\times n \times n}$ and $(a\otimes b\otimes b)_{ijk}=a_ib_jc_k$. The setting, we're interested in is similar to that for NMF -- consider 


==> lr_theory.tex <==
\subsection{Guarantees for linear classification}

\begin{restatable}{prop}{lr}\label{prop:lr}
	
\end{restatable}

==> nmf_app_old.tex <==
\section{Additional proofs for Section \ref{sec:nmf_theory}: Uniqueness for NMF}\label{sec:nmf_app}

\subsection{Proof of Part (a) of Theorem \ref{thm:nmf}}
\begin{proof}
	As in Part (b), we will argue about the row space of the matrix $H$. By the same argument as in Part (b) ,for any alternative factorization ${M}=W'H'$, the row space of $H'$ must equal the row space of $M$, which equals the row space of $H$. As the row space of $H'$ equals the row space of $H$, therefore $H'$ must lie in the row space of $H$. Hence our goal we will prove that the rows of $H$ are the sparsest vectors in the row space of $H$, which implies that for any other factorization $M={W'}{H'}$, $\lpnorm{H}{0}<\lpnorm{{H'}}{0}$. Lemma \ref{lem:exp1} shows that the number of columns which are have at least one zero entry in a subset $S$ of the rows of $H$ grows proportionately with the size of $S$.
	\begin{restatable}{lem}{exp}\label{lem:exp1}
		For any subset $S$ of the rows of $H$, define $N(S)$ to be the subset of the columns of $H$ which have a non-zero entry in at least one of the rows in $S$. Then for every subset $S$ of rows of $H$,  $|N(S)|\ge\min\{4|S|k/5,n/200\}$ with high probability.
	\end{restatable}
	\begin{proof}
		Consider a bipartite graph $G$ with $r$ nodes on the left part $U$ corresponding to the $r$ rows of $H$, and $n$ nodes on the right part $V$ corresponding to the $n$ columns or indices of each factor. The $i$th node in $U$ has an edge to $k$ nodes in $V$ corresponding to the non-zero indices of the $i$th row of $H$. Note that $|N(S)|$ is the neighborhood of the set of nodes $S$ in $G$. From Part 1 of Lemma \ref{expander}, the graph $G$ is a $(\gamma_1 r,4/5)$ expander with failure probability $re^{-\beta k}/n$ for $\gamma_1 = n/(rke^5)$ and a fixed constant $\beta>0$. 
		
		\begin{restatable}{lem}{expander}\label{expander}
			Randomly choose a bipartite graph $G$ with $n_1$ vertices on the left part $U$ and $n_2$ vertices on the right part $V$ such that every vertex in $U$ has degree $D$. Then,
			\begin{enumerate}
				\item  For every $n_1, n_2, n_1<n_2$, $G$ is a $(\gamma n_1, 4/5)$ expander for $D\ge c$ for some fixed constant $c$ and $\gamma n_1 =\frac{n_2}{De^{5}}$ except with probability $n_1e^{-\beta D}/n_2$ for a fixed constant $\beta>0$.
				\item For every $n_1, n_2, n_2 <n_1$, $G$ is a $(\gamma n_1, 4/5)$ expander for $D\ge c\log n_1$ for some fixed constant $c$ and $\gamma n_1 =\frac{n_2}{De^{5}}$ except with probability $1/n_2$.
			\end{enumerate}
		\end{restatable}
		
		As $G$ is a $(\gamma_1 r,4/5)$ expander, every set of $|S|\le \gamma_1 r$ nodes has at least $4|S|k/5$ neighbors. A set of size $|S| >\gamma_1 r$ nodes, must include a subset of size $\gamma_1 r$ which has $4n/(5e^5)\ge n/200$ neighbours, and hence every set of size $|S|>\gamma_1 r$ has at least $n/200$ neighbors. Therefore, for every subset of $S$ rows, $|N(S)|\ge\min\{4|S|k/5,n/200\}$ with failure probability $re^{-\beta k}/n$.
	\end{proof}
	
	We now show the second part of the proof---that for any subset $S$ of the rows, every linear combination of all $S$ rows  must have $|N(S)|-|S|$ non-zero entries. The following simple Lemma is a restatement of a result from from \citet{spielman2012exact}. We provide a proof in the appendix for completeness. Define a vector $x$ as \emph{fully dense} if all its entries are non-zero. 
	
	\begin{restatable}{lem}{nmfnulli}\label{lem:null1}
		Let $\Omega\in \{0,1\}^{n\times n}$ be any binary matrix with at least one nonzero in each column. Let $U=\Omega\odot Y$ where each entry of $Y$ is drawn independently from $N(0,1)$. Then with probability one in the random matrix $V$, the left nullspace of $U$ does not contain a fully dense vector.
	\end{restatable}
	\begin{proof}
		Let $\mathcal{N}_i$ be the null space of the first $i$ columns of $U$, we define $\mathcal{N}_0=\mathbb{R}^n$. We will show that with probability one, either $N_i$ does not contain a fully dense vector, or $\rank(\mathcal{N}_i)=n-i$. The proof proceeds by induction. Consider $i=1$. Consider any full dense vector $x \in \mathbb{R}^n$. As every column of $U$ has at least one non-zero entry, the probability that $x$ is orthogonal to the first column $U_1$ is exactly zero. This is because the non-zero entries of $U_1$ are independent Gaussian random variables, hence the probability that any fixed linear combination is zero is exactly zero. Hence $\rank(\mathcal{N}_1)=\rank(\mathcal{N}_0)-1=n-1$ with probability 1. Consider the $j$th step. By the induction hypothesis, either $\mathcal{N}_j$ does not contain any fully dense vector, or $\rank(\mathcal{N}_{j})=n-j$. If $\mathcal{N}_j$ does not contain any fully dense vector, then we are done as this implies that $\mathcal{N}_{j+1}$ also does not contain a fully dense vector. Let $\mathcal{N}_j$ contain a fully dense vector $x$. The $(j+1)$th column $U_{j+1}$ of $U$ has at least one non-zero entry, and the entries are independent of the previous columns. The probability that $x$ is orthogonal to $U_{j+1}$ is  zero, by the previous argument. Hence with probability one, either $\mathcal{N}_{j+1}$ does not contain a fully dense vector, or $\rank(\mathcal{N}_{j+1})=\rank(\mathcal{N}_{j+1})-1=n-j-1$. This proves the induction argument. Therefore, with probability 1, either  $\rank(\mathcal{N}_{n})=0$ or $\mathcal{N}_n$ does not contain a fully dense vector. Hence the left null space of $U$ does not contain a fully dense vector.
	\end{proof}
	
	We now complete the proof for the first part of Theorem \ref{thm:nmf}. Consider any set $S$ of the rows of $H$.  Consider any linear combination $v\in \mathbb{R}^n$ of the set $S$ rows, such that all the combination weights $x\in\mathbb{R}^{|S|}$ are non-zero. By Lemma \ref{lem:exp1}, $|N(S)|\ge \min\{4|S|k/5,n/200\}$ with failure probability $re^{-\beta k}/n$. We claim that $v$ has more than $|N(S)|-|S|$ non zero entries. We prove by contradiction. Assume that $v$ has at most $|N(S)|-|S|$ non zero entries. Consider the submatrix $U$ of $H$ corresponding to the $S$ rows and $N(S)$ columns. If $v$ has $|N(S)|-|S|$ or fewer non zero entries, then there must be a subset $S'$ of the $|N(S)|$ columns of $U$ with $|S'|=|S|$, each of which has at least one non-zero entry, and such that the fully dense vector $x$ lies in the left null space of $S'$. But by Lemma \ref{lem:null1}, the probability of this happening is zero. Hence $v$ has more than $|N(S)|-|S|$ non zero entries. Note that $|N(S)|-|S|\ge  7 k/5$. Hence any linear combination of more than one row of $H$ has more than $7k/5$ non-zero entries with failure probability $re^{-\beta k}/n$. Hence the rows of $H$ are the sparsest vectors in the row space of $H$ with failure probability $re^{-\beta k}/n$.
\end{proof}

\subsection{Additional proofs for Part (b) of Theorem \ref{thm:nmf}}

Lemma \ref{lem:exp2} shows that the number of columns which are have at least one zero entry in a subset $S$ of the columns of $W$ columns proportionately with the size of $S$. The proof proceeds by showing that choosing $B$ such that each column has $k$ randomly chosen non-zero entries ensures expansion for $B$ with high probability, and the fact that $P$ is given to be an expander.
\vspace{-5pt}
\begin{restatable}{lem}{expii}\label{lem:exp2}
	For any subset $S$ of the columns of $\tilde{W}$, define $N(S)$ to be the subset of the columns of $\tilde{W}$ which have a non-zero entry in at least one of the columns in $S$. Then for every subset $S$ of columns of $\tilde{W}$,  $|N(S)|\ge\min\{16|S|kp/25,d/200\}$ with failure probability $re^{-\beta k}/n$.
\end{restatable}
\vspace{-8pt}
We now prove the second part of the argument--that any linear combination of columns in $S$ cannot have much fewer non-zero entries than $N(S)$, as the probability that many of the non-zero entries get canceled is zero. Lemma \ref{lem:null2} is the key to showing this. Define a vector $x$ as \emph{fully dense} if all its entries are non-zero.
\vspace{-5pt}
\begin{lem}\label{lem:null2}
	For any subset $S$ of the columns of $\tilde{W}$, let $U$ be the submatrix of $\tilde{W}$ corresponding to the $S$ columns and $N(S)$ columns. Then with probability one, every subset of the columns of $U$ of size at least $|S|p$ does not have any fully dense vector in its left null space. 
\end{lem}
\vspace{-15pt}
\begin{proof}
	Without loss of generality, assume that $S$ corresponds to the first $|S|$ columns of $\tilde{W}$, and $N(S)$ corresponds to the first $|N(S)|$ columns of $\tilde{W}$. We will partition the columns of $U$ into $|S|$ groups $\{\mathcal{G}_1,\dots, \mathcal{G}_{|S|}\}$. Each group will have size at most $p$. To select the first group, we choose any entry $y_1$ of $Y$ which appears in the first row of $U$. For example, if the first column of $W$ has a one in its first row, and $P(1,1)=1$, then the random variable $Y_{1,1}$ appears in the first row of $U$. Say we choose $y_1=Y_{1,1}$. We then choose $\mathcal{G}_1$ to be the set of all columns where $y_1$ appears. We then remove the set of columns $\mathcal{G}_1$ from $U$. To select the second group, we pick any one of the remaining columns, and choose any entry $y_2$ of $Y$ which appears in that row of $U$. $\mathcal{G}_2$ is the set of all columns where $y_2$ appears. We repeat this procedure to obtain $|S|$ groups, each of which will have size at most $p$ as every variable appears in $p$ columns.
	
	% Consider the first row $U_1$ of $U$. Consider any fully dense vector $x\in\mathbb{R}^{|S|}$. As $U_1$ contains at least one non-zero entry, with probability one over the randomness in the entries of $U_1$, $x$ is not orthogonal to $U_1$. Choose any entry $y_1$ of the matrix $Y$ which appears in the row $U_1$. The set of all columns in which $y_1$ appears comprise our first group $\mathcal{G}_1$ of columns. We have shown that $\rank(\mathcal{N}_1)=\rank(\mathcal{N}_0)-1=t-1$.
	Let $\mathcal{N}_j$ be the left null space of the first $j$ groups of columns. We define $\mathcal{N}_0=\mathbb{R}^{|S|}$. We will now show that either $\rank(\mathcal{N}_i)=|S|-i$ or $\mathcal{N}_i$ does not contain a fully dense vector. We prove this by induction. Consider the $j$th step, at which we have $j$ groups $\{\mathcal{G}_1, \dots, \mathcal{G}_j\}$. By the induction hypothesis, either $\mathcal{N}_j$ does not contain any fully dense vector,  or $\rank(\mathcal{N}_j)=|S|-j$. If $\mathcal{N}_j$ does not contain any fully dense vector, then we are done as this implies that $\mathcal{N}_{j+1}$ also does not contain any fully dense vector. Assume that  $\mathcal{N}_j$ contains a fully dense vector $x$. Choose any row $U_c$ which has not been already been assigned to one of the sets. By the following elementary proposition, the probability that $x$ is orthogonal to $U_c$ is zero. We provide a proof in the appendix.
	\begin{restatable}{prop}{ele}
		Let $v=(v_1,\dots,v_n)\in \mathbb{R}^n$ be a vector of $n$ independent $N(0,1)$ random variables. For any subset $S\subseteq \{1,\dots,n\}$, let $v(S)\in\mathbb{R}^{|S|}$ refer to the subset of $v$ corresponding to the indices in $S$. Consider $t$ such subsets $S_1,\dots, S_t$. Let each set $S_i$ defines some linear relation $\alpha_{S_i}^Tv(S_i)=0$, for some $\alpha_{S_i}\in \mathbb{R}^{|S_i|}$. Assume that the variable $v_{i}$ appear in the set $S_i$. Then the probability distribution of the set of variables $\{v_{t+1},\dots,v_{n}\}$ conditioned on the linear relations defined by $S_1,\dots, S_t$ is still continuous and its density function has full support. In particular, any linear combination of the set of variables $\{v_{t+1},\dots,v_{n}\}$ has zero probability of being zero.
	\end{restatable}
	\vspace{-5pt}
	If $\mathcal{N}_{j}$ contains a fully dense vector, then with probability one, $\rank(\mathcal{N}_{j+1})=\rank(\mathcal{N}_{j})-1=n-j-1$. This proves the induction argument. Therefore, with probability one, either  $\rank(\mathcal{N}_{|S|})=0$ or $\mathcal{N}_{|S|}$ does not contain a fully dense vector and Lemma \ref{lem:null2} follows. %Hence the left nullspace of $U$ does not contain a fully dense vector.
\end{proof}
\vspace{-10pt}
We now complete the proof for the second part of Theorem \ref{thm:nmf}. Note that the columns of $\tilde{W}$ have at most $kp$ non-zero entries. Consider any set $S$ of columns of $\tilde{W}$.  Consider any linear combination $v\in \mathbb{R}^d$ of the set $S$ columns, such that all the combination weights $x\in\mathbb{R}^{|S|}$ are non-zero. By Lemma \ref{lem:exp2}, $|N(S)|\ge \min\{16|S|kp/25,d/200\}$ with failure probability $re^{-\beta k}/n$. We claim that $v$ has more than $|N(S)|-|S|p$ non zero entries. We prove by contradiction. Assume that $v$ has $|N(S)|-|S|$ or fewer non zero entries. Consider the submatrix $U$ of $\tilde{W}$ corresponding to the $S$ columns and $N(S)$ columns. If $v$ has $|N(S)|-|S|p$ or fewer non zero entries, then there must be a subset $S'$ of the $|N(S)|$ columns of $U$ with $|S'|=|S|p$, such that each of the columns in $S'$ has at least one non-zero entry, and the fully dense vector $x$ lies in the left null space of $S'$. But by Lemma \ref{lem:null2}, the probability of this happening is zero. Hence $v$ has more than $|N(S)|-|S|p$ non zero entries. Lemma \ref{lem:nmf_comp} obtains a lower bound on $|N(S)|-|S|p$ using simple algebra.
\begin{restatable}{lem}{nmfcom}\label{lem:nmf_comp}
	$|N(S)|-|S|p \ge 6kp/5$ for $|S|>1$ for $d\ge 400p(r+k)$.
\end{restatable}
\vspace{-10pt}	
Hence any linear combination of more than one column of $\tilde{W}$ has at least $6kp/5$ non-zero entries with failure probability $re^{-\beta k}/n$. Hence the columns of $\tilde{W}$ are the sparsest vectors in the column space of $\tilde{W}$ with failure probability $re^{-\beta k}/n$.

\expii*
\begin{proof}
	Recall that in the proof of Lemma \ref{lem:exp1}, we considered a bipartite graph corresponding to the $r$ rows and the $n$ indices. After the projection step, the $n$ indices are projected to $d$ dimensions, and the projection matrix is a $(\gamma_2 n, 4/5)$ expander with $\gamma_2 = d/(nke^5)$. We can now consider a tripartite graph, by adding a third set $W$ with $d$ nodes. We add an edge from a node $i$ in $V$ to node $j$ in $W$ if $P(j,i)=1$. For any subset $S$ of rows of $\tilde{H}$, $N(S)$ are the set of nodes in $W$ which are reachable from the nodes $S$ in $U$. By Lemma \ref{lem:exp1}, the number of neighbors in $V$ of any set $S$ of nodes in $U$ is of size at least $\min\{4|S|k/5,n/200\}$ with failure probability $re^{-\beta k}/n$. As the projection matrix $P$ is a $(\gamma_2 n, 4/5)$ expander with $\gamma_2 = d/(npe^5)$, every subset of size $t$ in $V$ has at least $\min\{4tp/5,d/200\}$ neighbors in $W$. By combining this argument with Lemma \ref{lem:exp1}, it follows that for every subset of $S$ rows of $H$,  $|N(S)|\ge\min\{16|S|kp/25,d/200\}$ with failure probability $re^{-\beta k}/n$..
\end{proof}


\ele*
\begin{proof}
	We prove by induction. For the base case, note that without any linear constraints, the set of $n$ random variables $\{v_{1},\dotsb,v_{n}\}$ is continuous and has full support as the random variables $v_i$ are independent Gaussian. Consider the $j$th step, when linear constraints defined by the sets $S_1,\dotsb,S_{j}$ have been imposed on the variables. We claim that the distribution of the set of random variables $\{v_{j+1},\dotsb,v_{n}\}$ is continuous and has full support after imposition of the constraints $S_1,\dotsb,S_j$. By the induction hypothesis, the distribution of the set of random variables $\{v_{j},\dotsb,v_{n}\}$ is continuous and has full support after imposition of the constraints $S_1,\dotsb,S_{j-1}$. Note that the linear constraint $S_j$ can be satisfied for any assignment to the subset of  variables $\{v_{j+1},\dotsb,v_{n}\}$ which appear in the constraint $S_j$, as $v_j$ can be chosen appropriately because by the induction hypothesis it has full support conditioned on the previous constraints $S_1,\dotsb, S_{j-1}$. Hence the probability distribution of the set of variables $\{v_{j+1},\dotsb,v_{n}\}$ is still continuous and has full support after adding the constraint $S_j$.
\end{proof}

\nmfcom*
\begin{proof}
	For $2\le |S|\le  d/(128kp)$, 
	\begin{align}
	|N(S)|-|S|p&\ge (16kp/25)|S|-p|S|=30kp/25+kp(16|S|-30)/25-p|S| \nonumber\\
	&\ge 6kp/5+p\Big(k(16|S|-30)-|S|\Big) \nonumber
	\end{align} 
	For $|S|\ge 2$ and $k\ge2$, $k(16|S|-30)-|S|\ge 0$, hence $|N(S)|-|S|p\ge 6kp/5$ for $2\le |S|\le  d/(128kp)$. For $|S|>d/(128kp)$, $|N(S)|\ge d/200$. Therefore, $|N(S)|-|S|p\ge d/200-rp\ge 2kp$ for $d\ge 400p(r+k)$. 
\end{proof}

\spaceeq*
	\begin{proof}
		Note that the column space of $\tilde{M}$ is a subspace of the column space of $\tilde{W}$. As $H$ is full row rank, the rank of the column space of $\tilde{M}$ equals the rank of the column space of $\tilde{W}$. Therefore, the column space of $\tilde{M}$ equals the column space of $\tilde{W}$. By the same argument, for any alternative factorization $\tilde{M}=W'H'$, the column space of $W'$ must equal the column space of $\tilde{M}$---which equals the column space of $\tilde{W}$. As the column space of $W'$ equals the column space of $\tilde{W}$, therefore $W'$ must lie in the column space of $\tilde{W}$.
	\end{proof}

==> nmf_syn.tex <==
\subsection{NMF experiments on synthetic data}

\begin{figure}[h]
	\centering
	\begin{subfigure}{0.4 \textwidth}
		\includegraphics[height=1.5in]{time_sim}
		\caption{Time taken for solving NMF in original space and compressed space}
		\label{fig:nmf_sim1}
	\end{subfigure}
	\begin{subfigure}{0.4 \textwidth}
		\includegraphics[height=1.5 in]{q_sim}
		\caption{Quality of solution for solving NMF in original space and compressed space}
		\label{fig:nmf_sim2}
	\end{subfigure}
	\caption{Synthetic experiments on NMF. The total number of non zero entries per row of $H$ is fixed to be $k=20$ and rank $r=20$. We project down to $k\log n$ dimensions. We obtain significant asymptotic speedups with negligible change in accuracy in this case.}
	\label{fig:nmf_sim}
\end{figure}

We perform experiments on NMF using synthetic data where we can control the sparsity of the true factors to verify how our approach performs if the factors are very sparse. We take $n=m$ and $r=20$. We vary $n$ from 1000 to 10000. For $M=WH$, we set $W$ to be the absolute value of a matrix $G\in \mathbb{R}^{n\times r}$ such that the entries of $G$ are independent Gaussian random variables. For each row of $H$, we fix the number of non-zero entries to be $k=20$. We project down to the theoretical limit of $d=O(k\log n)$. We can see from Fig. \ref{fig:nmf_sim1} and \ref{fig:nmf_sim2} that we can get significant speedups in this setting, at negligible degradation in accuracy. Of course, this setting is highly artificial, but serves as a sanity check that compressed NMF works.

==> nmf_theory_old.tex <==
\section{Guarantees for our approach}\label{sec:theory}

In this section, we will show uniqueness guarantees for performing non-negative matrix factorization and tensor decomposition on the projected matrix. This will establish that the factors in the projected space correspond to a projection of the factors in the original space. %We believe it is possible to show similar guarantees for linear classification, using results on the quality of 

\subsection{Guarantees for Non-negative matrix factorization}

\citet{donoho2004does} showed that non-negative matrix factorization is unique under the separability condition, subsequently \citet{arora2012computing} also showed that NMF can be computed efficiently under this condition. However, separability can be a very strong condition in practice. Instead of using separability, we desire to obtain uniqueness results for NMF using sparsity of the weight matrix $H$. Our uniqueness results in the original space are similar in principle to uniqueness results obtained for sparse coding by \citet{spielman2012exact}. We show that if a matrix $M$ has a true rank $r$ factorization $M=WH$ and $H$ is sparse, then for any other rank $r$ factorization $M=W'H'$. $H'$  has strictly more non-zero entries than $H$. As NMF has been found to recover sparse solutions, and there are algorithms which explicitly enforce sparsity \cite{hoyer2004non}, it is reasonable to hope that the recovery procedure will be successful if the true solution is the sparsest possible solution. The main technical challenge of proving Theorem \ref{thm:nmf} is in the projected space. This is because in the original space we could use the fact the entries of $H$ are drawn independently at random to greatly simplify our arguments, however we lose access to this independence after the random projection step. The proof in the projected space crucially uses the expansion properties of the projection matrix $P$ to get around this, enabling us to prove similar uniqueness results in the projected space.  % Recently, \citet{li2016recovery} obtained local convergence guarantees for the alternating minimization approach to NMF. They only used the fact that 

\begin{thm}\label{thm:nmf}
	Consider a rank $r$ matrix $M\in \mathbb{R}^{m\times n}$ which has factorization $M=WH$ where $W\in \mathbb{R}^{m\times r}$ is full column rank, $H\in \mathbb{R}^{r\times n}$ and $H=B \odot Y$ where each row row of $B$ has exactly $k$ non-zero entries chosen uniformly at random and each entry of $Y$ is drawn independently from $N(0,1)$. Assume $k>C$, where $C$ is a fixed constant. Consider the projection matrix $P\in \{0,1\}^{n\times d}$ where each row of $P$ has exactly $p$ non-zero entries, $p=O(\log n)$ and $P$ is a $(\gamma n, 4/5)$ expander with $\gamma=d/(npe^5)$ . Assume $d=\Omega(p(r+k))$. Let $\tilde{M}=MP$. Note that $\tilde{M}$ has a factorization $\tilde{M}=W\tilde{H}$ where $\tilde{H}=HP$. Then,
	\begin{enumerate}[(a)]
		\item For any other rank $r$ factorization $M={W'}{H'}$, $\lpnorm{H}{0}<\lpnorm{{H'}}{0}$ with failure probability at most $re^{-\beta k}/n$ for some $\beta>0$.
		\item For any other rank $r$ factorization $\tilde{M}={W'}{H'}$, $\lpnorm{\tilde{H}}{0}<\lpnorm{{H'}}{0}$ with failure probability at most $re^{-\beta k}/n$ for some $\beta>0$.
	\end{enumerate}  
\end{thm}
\begin{proof}	
	We prove Part (a) of Theorem \ref{thm:nmf} in the Appendix. Here, we provide the outline of the proof for the more challenging Part (b). We will argue about the row space of the matrix $H$. We first claim that the row space of $M$ equals the row space of $H$. To verify, note that the row space of $M$ is a subspace of the row space of $H$. As $W$ is full column rank, the rank of the row space of $M$ equals the rank of the row space of $H$. Therefore, the row space of $M$ equals the row space of $H$. By the same argument, for any alternative factorization ${M}=W'H'$, the row space of $H'$ must equal the row space of $M$, which equals the row space of $H$. As the row space of $H'$ equals the row space of $H$, therefore $H'$ must lie in the row space of $H$. Hence our goal we will prove that the rows of $H$ are the sparsest vectors in the row space of $H$, which implies that for any other factorization $M={W'}{H'}$, $\lpnorm{H}{0}<\lpnorm{{H'}}{0}$.

The outline of the proof is as follows. First, we argue that the if we take any subset $S$ of the rows of $H$, then the number of columns which have non-zero entries in any of the rows in $S$ is large. This implies that taking a linear combination of all the $S$ rows will result in a vector with a large number of non-zero entries---unless the non-zero entries cancel in many of the columns. But this happens with zero probability, as the non-zero entries of $H$ are independent Gaussian random variables, and the probability that they take on any specific value is exactly zero. 

Lemma \ref{lem:exp1} shows that the number of columns which are have at least one zero entry in a subset $S$ of the rows of $H$ grows proportionately with the size of $S$.
\begin{restatable}{lem}{exp}\label{lem:exp1}
	For any subset $S$ of the rows of $H$, define $N(S)$ to be the subset of the columns of $H$ which have a non-zero entry in at least one of the rows in $S$. Then for every subset $S$ of rows of $H$,  $|N(S)|\ge\min\{4|S|k/5,n/200\}$ with high probability.
\end{restatable}

We now show the second part of the proof---that for any subset $S$ of the rows, every linear combination of all $S$ rows  must have $|N(S)|-|S|$ non-zero entries. The following simple Lemma is a restatement of a result from from \citet{spielman2012exact}. We provide a proof in the appendix for completeness. Define a vector $x$ as \emph{fully dense} if all its entries are non-zero. 

\begin{restatable}{lem}{nmfnulli}\label{lem:null1}
	Let $\Omega\in \{0,1\}^{n\times n}$ be any binary matrix with at least one nonzero in each column. Let $U=\Omega\odot Y$ where each entry of $Y$ is drawn independently from $N(0,1)$. Then with probability one in the random matrix $V$, the left nullspace of $U$ does not contain a fully dense vector.
\end{restatable}

We now complete the proof for the first part of Theorem \ref{thm:nmf}. Consider any set $S$ of the rows of $H$.  Consider any linear combination $v\in \mathbb{R}^n$ of the set $S$ rows, such that all the combination weights $x\in\mathbb{R}^{|S|}$ are non-zero. By Lemma \ref{lem:exp1}, $|N(S)|\ge \min\{4|S|k/5,n/200\}$ with failure probability $re^{-\beta k}/n$. We claim that $v$ has more than $|N(S)|-|S|$ non zero entries. We prove by contradiction. Assume that $v$ has at most $|N(S)|-|S|$ non zero entries. Consider the submatrix $U$ of $H$ corresponding to the $S$ rows and $N(S)$ columns. If $v$ has $|N(S)|-|S|$ or fewer non zero entries, then there must be a subset $S'$ of the $|N(S)|$ columns of $U$ with $|S'|=|S|$, each of which has at least one non-zero entry, and such that the fully dense vector $x$ lies in the left null space of $S'$. But by Lemma \ref{lem:null1}, the probability of this happening is zero. Hence $v$ has more than $|N(S)|-|S|$ non zero entries. Note that $|N(S)|-|S|\ge  7 k/5$. Hence any linear combination of more than one row of $H$ has more than $7k/5$ non-zero entries with failure probability $re^{-\beta k}/n$. Hence the rows of $H$ are the sparsest vectors in the row space of $H$ with failure probability $re^{-\beta k}/n$.

\emph{Part (b):} As $d\ge r$, we can repeat our previous argument to show that for any other factorization $\tilde{M}=W{H'}$, the row space of ${H'}$ must be the same as the row space of $\tilde{H}$. The proof proceeds as before--we will show that rows of $\tilde{H}$ are the sparsest vectors in the row space of $\tilde{H}$. We begin the proof by showing that for any subset $S$ of the rows of $\tilde{H}$, Lemma \ref{lem:exp2} shows that $|N(S)|$ grows proportionately with the size of $S$. The proof is similar to the proof of Lemma \ref{lem:exp1} and is given in the appendix.

\begin{restatable}{lem}{exp}\label{lem:exp2}
	For any subset $S$ of the rows of $\tilde{H}$, define $N(S)$ to be the subset of the columns of $\tilde{H}$ which have a non-zero entry in at least one of the rows in $S$. Then for every subset $S$ of rows of $\tilde{H}$,  $|N(S)|\ge\min\{16|S|kp/25,d/200\}$ with failure probability $re^{-\beta k}/n$..
\end{restatable}

We now prove the second part of the argument--that any linear combination of $S$ rows cannot have much fewer non-zero entries than $N(S)$, as the probability that many of the non-zero entries get canceled is zero. Lemma \ref{lem:null2} is the key to showing this, and is analogous to Lemma \ref{lem:null1} in the Part (a).

\begin{lem}\label{lem:null2}
	For any subset $S$ of the rows of $\tilde{H}$, let $N(S)$ be the subset of columns of the columns of $\tilde{H}$ which have a non-zero entry in at least one of the rows in $S$. Let $U$ be the submatrix of $\tilde{H}$ corresponding to the $S$ rows and $N(S)$ columns. Then with probability one, every subset of the columns of $U$ of size at least $|S|p$ does not have any fully dense vector in its left null space. 
\end{lem}
\begin{proof}
	Without loss of generality, assume that $S$ corresponds to the first $|S|$ rows of $\tilde{H}$, and $N(S)$ corresponds to the first $|N(S)|$ columns of $\tilde{H}$. We will partition the columns of $U$ into $|S|$ groups $\{\mathcal{G}_1,\dotsb, \mathcal{G}_{|S|}\}$. Each group will have size at most $p$. To select the first group, we choose any entry $y_1$ of $Y$ which appears in the first column of $U$. For example, if the first row of $H$ has a one in its first column, and $P(1,1)=1$, then the random variable $Y_{1,1}$ appears in the first column of $U$. Say we choose $y_1=Y_{1,1}$. We then choose $\mathcal{G}_1$ to be the set of all columns where $y_1$ appears. We then remove the set of columns $\mathcal{G}_1$ from $U$. To select the second group, we pick any one of the remaining columns, and choose any entry $y_2$ of $Y$ which appears in that column of $U$. $\mathcal{G}_2$ is the set of all columns where $y_2$ appears. We repeat this procedure to obtain $|S|$ groups, each of which will have size at most $p$ as every variable appears in $p$ columns.
	
	 Let $\mathcal{N}_j$ be the left null space of the first $j$ groups of columns. We define $\mathcal{N}_0=\mathbb{R}^{|S|}$. Consider the first column $U_1$ of $U$. Consider any fully dense vector $x\in\mathbb{R}^{|S|}$. As $U_1$ contains at least one non-zero entry, with probability one over the randomness in the entries of $U_1$, $x$ is not orthogonal to $U_1$. Choose any entry $y_1$ of the matrix $Y$ which appears in the column $U_1$. The set of all columns in which $y_1$ appears comprise our first group $\mathcal{G}_1$ of columns. We have shown that $\rank(\mathcal{N}_1)=\rank(\mathcal{N}_0)-1=t-1$. We will now show that either $\rank(\mathcal{N}_i)=t-i$ or $\mathcal{N}_i$ does not contain a fully dense vector. We prove this by induction. Consider the $j$th step, at which we have $j$ groups $\{\mathcal{G}_1, \dotsb, \mathcal{G}_j\}$. By the induction hypothesis, either $\mathcal{N}_j$ does not contain any fully dense vector,  or $\rank(\mathcal{N}_j)=|S|-j$. If $\mathcal{N}_j$ does not contain any fully dense vector, then we are done as this implies that $\mathcal{N}_{j+1}$ also does not contain any fully dense vector. Assume that  $\mathcal{N}_j$ contains a fully dense vector $x$. Choose any column $U_c$ which has not been already been assigned to one of the sets. By the following elementary proposition, the probability that $x$ is orthogonal to $U_c$ is zero. We provide a proof in the appendix.
	 \begin{restatable}{prop}{ele}
	 	Let $v=(v_1,\dotsb,v_n)\in \mathbb{R}^n$ be a vector of $n$ independent $N(0,1)$ random variables. For any subset $S\subseteq \{1,\dotsb,n\}$, let $v(S)\in\mathbb{R}^{|S|}$ refer to the subset of $v$ corresponding to the indices in $S$. Consider $t$ such subsets $S_1,\dotsb, S_t$. Each set $S_i$ defines some linear relation $\alpha_{S_i}^Tv(S_i)=0$, for some $\alpha_{S_i}\in \mathbb{R}^{|S_i|}$. Assume that the variable $v_{i}$ appear in the set $S_i$. Then the probability distribution of the set of variables $\{v_{t+1},\dotsb,v_{n}\}$ conditioned on the linear relations defined by $S_1,\dotsb, S_t$ is still continuous and its density function has full support. In particular, any linear combination of the set of variables $\{v_{t+1},\dotsb,v_{n}\}$ has zero probability of being zero.
	 \end{restatable}
	 Hence if $\mathcal{N}_{j}$ contains a fully dense vector, then with probability one, $\rank(\mathcal{N}_{j+1})=\rank(\mathcal{N}_{j})-1=n-j-1$. This proves the induction argument. Hence with probability one, either  $\rank(\mathcal{N}_{|S|})=0$ or $\mathcal{N}_{|S|}$ does not contain a fully dense vector. Hence the left nullspace of $U$ does not contain a fully dense vector.
\end{proof}
We now complete the proof for the second part of Theorem \ref{thm:nmf}. Note that the rows of $\tilde{H}$ have at most $kp$ non-zero entries. Consider any set $S$ of rows of $\tilde{H}$.  Consider any linear combination $v\in \mathbb{R}^d$ of the set $S$ rows, such that all the combination weights $x\in\mathbb{R}^{|S|}$ are non-zero. By Lemma \ref{lem:exp2}, $|N(S)|\ge \min\{16|S|kp/25,d/200\}$ with failure probability $re^{-\beta k}/n$. We claim that $v$ has more than $|N(S)|-|S|p$ non zero entries. We prove by contradiction. Assume that $v$ has $|N(S)|-|S|$ or fewer non zero entries. Consider the submatrix $U$ of $H$ corresponding to the $S$ rows and $N(S)$ columns. If $v$ has $|N(S)|-|S|p$ or fewer non zero entries, then there must be a subset $S'$ of the $|N(S)|$ columns of $U$ with $|S'|=|S|p$, such that each of the columns in $S'$ has at least one non-zero entry, and the fully dense vector $x$ lies in the left null space of $S'$. But by Lemma \ref{lem:null2}, the probability of this happening is zero. Hence $v$ has more than $|N(S)|-|S|p$ non zero entries. For $2\le |S|\le  d/(128kp)$, \begin{align}
|N(S)|-|S|p&\ge (16kp/25)|S|-p|S|=30kp/25+kp(16|S|-30)/25-p|S| \nonumber\\
&\ge 6kp/5+p\Big(k(16|S|-30)-|S|\Big)
\end{align} 
For $|S|\ge 2$ and $k\ge2$, $k(16|S|-30)-|S|\ge 0$, hence $|N(S)|-|S|p\ge 6kp/5$ for $2\le |S|\le  d/(128kp)$. For $|S|>d/(128kp)$, $|N(S)|\ge d/200$. Therefore, $|N(S)|-|S|p\ge d/200-rp\ge 2kp$ for $d\ge 400p(r+k)$. 

Hence any linear combination of more than one row of $\tilde{H}$ has at least $6kp/5$ non-zero entries with failure probability $re^{-\beta k}/n$. Hence the rows of $\tilde{H}$ are the sparsest vectors in the row space of $\tilde{H}$ with failure probability $re^{-\beta k}/n$.

\end{proof}


==> nmf_theory_old2.tex <==
\section{Guarantees for our approach}\label{sec:theory}

In this section, we will show uniqueness guarantees for performing non-negative matrix factorization and tensor decomposition on the projected matrix or tensor. This will establish that the factors in the projected space correspond to a projection of the factors in the original space, a prerequisite for being able to use compressive sensing to recover the factors in the original space.  %We believe it is possible to show similar guarantees for linear classification, using results on the quality of 

\subsection{Guarantees for non-negative matrix factorization}\label{sec:nmf_theory}

The known uniqueness guarantees for NMF are under the strong structural assumption of \emph{separability} , under which all the columns of the matrix are convex combinations of only a small set of columns \cite{donoho2004does}. However, in our compressed factorization setup we only know that the underlying factors are \emph{sparse}, and they need not be separable. Hence our goal in this section is to show uniqueness guarantees for NMF after random projection under sparsity assumptions on the underlying factors. We will first provide a summary of the result and discuss the underlying assumptions, then state the theorem formally with a proof sketch. 

We now describe our uniqueness results for NMF under random projections. Consider a matrix $M$ which has a rank $r$ non-negative factorization $M=WH$, and $W$ is sparse. Let $\tilde{W}=PW$ be the projection of $W$, and $\tilde{M}=PM$ be the projection of $M$. We show that for a suitable projection matrix $P$, with high probability $\tilde{M}=\tilde{W}H$ is the \emph{sparsest} possible factorization of $\tilde{M}$ in the following sense---for any other factorization $\tilde{M}={W}'H'$, $W'$ has strictly more non-zero entries than $\tilde{W}$. A guarantee of this nature is relevant in our regime as we are interested in sparse factorizations. Though we do not directly show that $\tilde{M}=\tilde{W}H$ is the unique non-negative factorization of the projected matrix $\tilde{M}$, but NMF has been found to recover sparse solutions \cite{lee1999learning,hoyer2004non}, and sparsity is often explicitly enforced in popular algorithms for NMF \cite{hoyer2004non}, hence our results provide compelling evidence that NMF in the projected space recovers the projection of the original factorization, i.e. $\tilde{M}=\tilde{W}H$. In this respect of providing guarantees for uniqueness of a sparse representation of a matrix, our result also applies to and extends guarantees for the \emph{sparse coding} problem \cite{spielman2012exact}.


% in fact obtaining sparse factorizations it is reasonable to hope that the recovery procedure will be successful if the true solution is the sparsest possible solution. The main contribution of Theorem \ref{thm:nmf} is Pa

%then for any other rank $r$ factorization $M=W'H'$, $H'$ has strictly more non-zero entries than $H$.

%Our uniqueness results for NMF using sparsity of the weight matrix $H$.


% showed that non-negative matrix factorization is unique under the \emph{separability} condition, under which all the columns of the matrix are convex combinations of only a small set of columns. This is very strong structural assumption separability is a very strong assumption, hence we  . Instead of using separability, we will show uniqueness results for NMF using sparsity of the weight matrix $H$. Our uniqueness results for NMF in the original space (Part (a) of Theorem \ref{thm:nmf}) are similar in principle to uniqueness results obtained for sparse coding by \citet{spielman2012exact}. We show that if a matrix $M$ has a true rank $r$ factorization $M=WH$ and $H$ is sparse, then for any other rank $r$ factorization $M=W'H'$, $H'$ has strictly more non-zero entries than $H$. As NMF has been found to recover sparse solutions \cite{lee1999learning,hoyer2004non}, and many algorithms explicitly enforce sparsity \cite{hoyer2004non}, it is reasonable to hope that the recovery procedure will be successful if the true solution is the sparsest possible solution. 

What projection matrices $P$ preserve uniqueness of NMF after random projections? We show that sparse--- binary matrices $P$, which are usually used as sensing matrices in the biomedical applications we consider---preserve uniqueness with high probability. The main property of such matrices which allows us to show uniqueness is that with high probability such matrices correspond to adjacency matrices of \emph{bipartite expander} graphs, we refer the reader to the proof sketch of Theorem \ref{thm:nmf} for the definition and properties of such graphs.

We now state Theorem \ref{thm:nmf}, and then discuss the quantitative bounds---

\begin{thm}\label{thm:nmf}
	Consider a rank $r$ matrix $M\in \mathbb{R}^{m\times n}$ which has factorization $M=WH$ where $W\in \mathbb{R}^{m\times r}$ is full column rank, $H\in \mathbb{R}^{r\times n}$ and $H=B \odot Y$ where each row of $B$ has exactly $k$ non-zero entries chosen uniformly at random, each entry of $Y$ is drawn independently from $N(0,1)$ \footnote{Note that the assumption that non-zero entries of $H$ are independent Gaussian random variables is not necessary and is stated for simplicity---any continuous probability distribution for the non-zero entries of $H$ suffices.} and $\odot$ denotes the element wise product. Assume $k>C$, where $C$ is a fixed constant. Consider the projection matrix $P\in \{0,1\}^{d\times n}$ where each column of $P$ has exactly $p$ non-zero entries with $p=O(\log n)$ and the $p$ non-zero entries in each column be chosen independently and uniformly at random. Assume $d=\Omega((r+k)\log n)$. Let $\tilde{M}=MP^T$. Note that $\tilde{M}$ has a factorization $\tilde{M}=W\tilde{H}$ where $\tilde{H}=HP^T$. Then, for any other rank $r$ factorization $\tilde{M}={W'}{H'}$, $\lpnorm{\tilde{H}}{0}<\lpnorm{{H'}}{0}$ with failure probability at most $re^{-\beta k}/n$ for some $\beta>0$.
%	\begin{enumerate}[(a)]
%		\vspace{-8pt}
%		\item For any other rank $r$ factorization $M={W'}{H'}$, $\lpnorm{H}{0}<\lpnorm{{H'}}{0}$ with failure probability at most $re^{-\beta k}/n$ for some $\beta>0$.
%		\vspace{-10pt}
%		\item For any other rank $r$ factorization $\tilde{M}={W'}{H'}$, $\lpnorm{\tilde{H}}{0}<\lpnorm{{H'}}{0}$ with failure probability at most $re^{-\beta k}/n$ for some $\beta>0$.
%	\end{enumerate}  
\end{thm}


%The main contribution of Theorem \ref{thm:nmf} is Part (b), which shows uniqueness results in the projected space. This is significantly more challenging than showing uniqueness in the original space, because in the original space we could use the fact the entries of $H$ are drawn independently at random to  simplify our arguments. However we lose access to this independence after the random projection step as the entries of the projected matrix are no longer independent. Instead, the proof in the projected space uses the expansion properties of the projection matrix $P$ to control the dependencies, enabling us to prove uniqueness results in the projected space. 

%Theorem \ref{thm:nmf} only assumes that $W$ is full column rank, and 
Theorem~\ref{thm:nmf} shows that if the rows of $H$ are $k$-sparse, then projecting into $\Omega(\log n(r+k))$ dimensions preserves uniqueness, with failure probability at most $e^{-\beta k}(r/n)$ for some constant $\beta>0$. The requirement for the projection dimension being at least $\Omega((r+k)\log n)$ seems necessary, as even being able to uniquely recover a $k$-sparse $n$-dimensional vector $x$ from its projection $Px$ requires the projection dimension to be at least $k\log n$.


\vspace{-12pt}
\begin{proof}	
	We prove Part (a) of Theorem \ref{thm:nmf} in Appendix \ref{sec:nmf_app}. Here, we provide the outline of the proof for the more challenging Part (b), moving proof details to Appendix \ref{sec:nmf_app}. We will argue about the row space of the matrix $\tilde{H}$. We first claim that the row space of $\tilde{M}$ equals the row space of $\tilde{H}$. To verify, note that the row space of $\tilde{M}$ is a subspace of the row space of $\tilde{H}$. As $W$ is full column rank, the rank of the row space of $\tilde{M}$ equals the rank of the row space of $\tilde{H}$. Therefore, the row space of $\tilde{M}$ equals the row space of $\tilde{H}$. By the same argument, for any alternative factorization $\tilde{M}=W'H'$, the row space of $H'$ must equal the row space of $\tilde{M}$ -- which equals the row space of $\tilde{H}$. As the row space of $H'$ equals the row space of $\tilde{H}$, therefore $H'$ must lie in the row space of $\tilde{H}$. Therefore, our goal will be to prove that the rows of $\tilde{H}$ are the sparsest vectors in the row space of $\tilde{H}$, which implies that for any other alternative factorization $\tilde{M}={W'}{H'}$, $\lpnorm{\tilde{H}}{0}<\lpnorm{{H'}}{0}$.

The outline of the proof is as follows. First, we argue that the if we take any subset $S$ of the rows of $\tilde{H}$, then the number of columns which have non-zero entries in at least one of the rows in $S$ is large. This implies that taking a linear combination of all the $S$ rows will result in a vector with a large number of non-zero entries---unless the non-zero entries cancel in many of the columns. But using the properties of the projection matrix $P$ and the fact that the non-zero entries of the original matrix $H$ are drawn from a continuous distribution, we show this happens with zero probability.

Lemma \ref{lem:exp2} shows that the number of columns which are have at least one zero entry in a subset $S$ of the rows of $H$ grows proportionately with the size of $S$. The proof proceeds by showing that choosing $B$ such that each row has $k$ randomly chosen non-zero entries ensures expansion for $B$ with high probability, and the fact that $P$ is given to be an expander.
\vspace{-5pt}
\begin{restatable}{lem}{expii}\label{lem:exp2}
	For any subset $S$ of the rows of $\tilde{H}$, define $N(S)$ to be the subset of the columns of $\tilde{H}$ which have a non-zero entry in at least one of the rows in $S$. Then for every subset $S$ of rows of $\tilde{H}$,  $|N(S)|\ge\min\{16|S|kp/25,d/200\}$ with failure probability $re^{-\beta k}/n$.
\end{restatable}
\vspace{-8pt}
We now prove the second part of the argument--that any linear combination of rows in $S$ cannot have much fewer non-zero entries than $N(S)$, as the probability that many of the non-zero entries get canceled is zero. Lemma \ref{lem:null2} is the key to showing this. Define a vector $x$ as \emph{fully dense} if all its entries are non-zero.
\vspace{-5pt}
\begin{lem}\label{lem:null2}
	For any subset $S$ of the rows of $\tilde{H}$, let $U$ be the submatrix of $\tilde{H}$ corresponding to the $S$ rows and $N(S)$ columns. Then with probability one, every subset of the columns of $U$ of size at least $|S|p$ does not have any fully dense vector in its left null space. 
\end{lem}
\vspace{-15pt}
\begin{proof}
	Without loss of generality, assume that $S$ corresponds to the first $|S|$ rows of $\tilde{H}$, and $N(S)$ corresponds to the first $|N(S)|$ columns of $\tilde{H}$. We will partition the columns of $U$ into $|S|$ groups $\{\mathcal{G}_1,\dots, \mathcal{G}_{|S|}\}$. Each group will have size at most $p$. To select the first group, we choose any entry $y_1$ of $Y$ which appears in the first column of $U$. For example, if the first row of $H$ has a one in its first column, and $P(1,1)=1$, then the random variable $Y_{1,1}$ appears in the first column of $U$. Say we choose $y_1=Y_{1,1}$. We then choose $\mathcal{G}_1$ to be the set of all columns where $y_1$ appears. We then remove the set of columns $\mathcal{G}_1$ from $U$. To select the second group, we pick any one of the remaining columns, and choose any entry $y_2$ of $Y$ which appears in that column of $U$. $\mathcal{G}_2$ is the set of all columns where $y_2$ appears. We repeat this procedure to obtain $|S|$ groups, each of which will have size at most $p$ as every variable appears in $p$ columns.
	
	% Consider the first column $U_1$ of $U$. Consider any fully dense vector $x\in\mathbb{R}^{|S|}$. As $U_1$ contains at least one non-zero entry, with probability one over the randomness in the entries of $U_1$, $x$ is not orthogonal to $U_1$. Choose any entry $y_1$ of the matrix $Y$ which appears in the column $U_1$. The set of all columns in which $y_1$ appears comprise our first group $\mathcal{G}_1$ of columns. We have shown that $\rank(\mathcal{N}_1)=\rank(\mathcal{N}_0)-1=t-1$.
	 Let $\mathcal{N}_j$ be the left null space of the first $j$ groups of columns. We define $\mathcal{N}_0=\mathbb{R}^{|S|}$. We will now show that either $\rank(\mathcal{N}_i)=|S|-i$ or $\mathcal{N}_i$ does not contain a fully dense vector. We prove this by induction. Consider the $j$th step, at which we have $j$ groups $\{\mathcal{G}_1, \dots, \mathcal{G}_j\}$. By the induction hypothesis, either $\mathcal{N}_j$ does not contain any fully dense vector,  or $\rank(\mathcal{N}_j)=|S|-j$. If $\mathcal{N}_j$ does not contain any fully dense vector, then we are done as this implies that $\mathcal{N}_{j+1}$ also does not contain any fully dense vector. Assume that  $\mathcal{N}_j$ contains a fully dense vector $x$. Choose any column $U_c$ which has not been already been assigned to one of the sets. By the following elementary proposition, the probability that $x$ is orthogonal to $U_c$ is zero. We provide a proof in the appendix.
	 \begin{restatable}{prop}{ele}
	 	Let $v=(v_1,\dots,v_n)\in \mathbb{R}^n$ be a vector of $n$ independent $N(0,1)$ random variables. For any subset $S\subseteq \{1,\dots,n\}$, let $v(S)\in\mathbb{R}^{|S|}$ refer to the subset of $v$ corresponding to the indices in $S$. Consider $t$ such subsets $S_1,\dots, S_t$. Let each set $S_i$ defines some linear relation $\alpha_{S_i}^Tv(S_i)=0$, for some $\alpha_{S_i}\in \mathbb{R}^{|S_i|}$. Assume that the variable $v_{i}$ appear in the set $S_i$. Then the probability distribution of the set of variables $\{v_{t+1},\dots,v_{n}\}$ conditioned on the linear relations defined by $S_1,\dots, S_t$ is still continuous and its density function has full support. In particular, any linear combination of the set of variables $\{v_{t+1},\dots,v_{n}\}$ has zero probability of being zero.
	 \end{restatable}
	 \vspace{-5pt}
	If $\mathcal{N}_{j}$ contains a fully dense vector, then with probability one, $\rank(\mathcal{N}_{j+1})=\rank(\mathcal{N}_{j})-1=n-j-1$. This proves the induction argument. Therefore, with probability one, either  $\rank(\mathcal{N}_{|S|})=0$ or $\mathcal{N}_{|S|}$ does not contain a fully dense vector and Lemma \ref{lem:null2} follows. %Hence the left nullspace of $U$ does not contain a fully dense vector.
\end{proof}
\vspace{-10pt}
We now complete the proof for the second part of Theorem \ref{thm:nmf}. Note that the rows of $\tilde{H}$ have at most $kp$ non-zero entries. Consider any set $S$ of rows of $\tilde{H}$.  Consider any linear combination $v\in \mathbb{R}^d$ of the set $S$ rows, such that all the combination weights $x\in\mathbb{R}^{|S|}$ are non-zero. By Lemma \ref{lem:exp2}, $|N(S)|\ge \min\{16|S|kp/25,d/200\}$ with failure probability $re^{-\beta k}/n$. We claim that $v$ has more than $|N(S)|-|S|p$ non zero entries. We prove by contradiction. Assume that $v$ has $|N(S)|-|S|$ or fewer non zero entries. Consider the submatrix $U$ of $\tilde{H}$ corresponding to the $S$ rows and $N(S)$ columns. If $v$ has $|N(S)|-|S|p$ or fewer non zero entries, then there must be a subset $S'$ of the $|N(S)|$ columns of $U$ with $|S'|=|S|p$, such that each of the columns in $S'$ has at least one non-zero entry, and the fully dense vector $x$ lies in the left null space of $S'$. But by Lemma \ref{lem:null2}, the probability of this happening is zero. Hence $v$ has more than $|N(S)|-|S|p$ non zero entries. Lemma \ref{lem:nmf_comp} obtains a lower bound on $|N(S)|-|S|p$ using simple algebra.
\begin{restatable}{lem}{nmfcom}\label{lem:nmf_comp}
	$|N(S)|-|S|p \ge 6kp/5$ for $|S|>1$ for $d\ge 400p(r+k)$.
\end{restatable}
\vspace{-10pt}	
	Hence any linear combination of more than one row of $\tilde{H}$ has at least $6kp/5$ non-zero entries with failure probability $re^{-\beta k}/n$. Hence the rows of $\tilde{H}$ are the sparsest vectors in the row space of $\tilde{H}$ with failure probability $re^{-\beta k}/n$.
\end{proof}


==> setup_old.tex <==
\section{Our Approach}
% Our approach consists of three simple steps. In the first step, we project down the original high dimensional optimization problem to low dimensions. In the second step, we solve the low dimensional optimization problem. In the third step, we use compressive sensing techniques to recover back the original solution to the high dimensional optimization problem from the solution to the low dimensional optimization problem. 
We instantiate our framework in the context of NMF and tensor decomposition.
In each case, we obtain a lower-dimensional problem via a random projection (described in detail in Sec.~\ref{sec:proj}). Denote the random projection matrix as $P\in \mathbb{R}^{d \times n}$, where $n$ is the original dimension and $d < n$. After solving the projected problem, we can obtain an approximation to the solution in the original space by solving a sparse recovery problem via the following linear program (LP):
\begin{equation}
\begin{aligned}
& \hat{w}^*= \underset{w}{\text{minimize}}
& & \|w\|_1,
& \text{subject to}
& & Pw = \tilde{w}^*
\end{aligned}
\label{eq:basis-pursuit}
\end{equation}
where $w \in \mathbb{R}^n$ and $\tilde{w}^* \in \mathbb{R}^d$ is the solution of the projected problem\footnote{In settings like NMF where the desired solution is non-negative, we can add the additional constraint $x \geq 0$ to Eq. \ref{eq:basis-pursuit}. In practice, we find that projecting the solutions of Eq. \ref{eq:basis-pursuit} post-hoc onto the non-negative orthant is often an effective heuristic. Omitting the additional constraint typically yields faster solution times.}. In the compressive sensing literature, this technique is also known as \emph{basis pursuit} \citep{chen2001atomic}. However, solving the LP can be computationally expensive, hence we will instead use efficient recovery algorithms which are much faster than solving the LP, but only work for sparse projection matrices. We describe how to choose the projection matrix next in Section \ref{sec:proj}, but first we will describe the specifics of each application of our method. %; it is well-known that the optimization problem can be recast as a linear program (LP) \citep{chen2001atomic}.

%\begin{enumerate}
	 \emph {Non-negative Matrix Factorization.} Consider the problem of factorizing a non-negative matrix $M\in \mathbb{R}^{m\times n}$ into a product of non-negative matrices $M=WH$. We are interested in the setting where matrix $H$ is sparse and $n\gg m$. We first project $M$ to $\tilde{M}=MP^T$. This corresponds to projecting each row of $H$ from $n$ dimensions to $d$ dimensions. We then factorize $\tilde{M}=\tilde{W}\tilde{H}$ by solving the NMF problem for $\tilde{M}$. We set our estimate $\hat{W}$ of $W$ to be $\tilde{W}$. To recover $H$ from $\tilde{H}$, we solve the compressive sensing problem in Eq. \ref{eq:basis-pursuit} for each row of $H_i$ of $H$. Therefore, for a rank-$r$ approximation, we solve $r$ instances of Eq. \ref{eq:basis-pursuit}. The outputs of the compressive sensing step are our estimates of the rows of $H$.
	 
	 \emph{Tensor decomposition.} The goal here is to decompose a tensor $T\in\mathbb{R}^{m_1 \times m_2 \times n}$ in terms of $r$ factors: $T=\sum_{i=1}^r A_i \otimes B_i \otimes C_i$ where $n\gg m_1,m_2$ and $C$ is sparse. We project the tensor $T$ along the 3rd mode to a projected tensor $\tilde{T}\in \mathbb{R}^{m_1 \times m_2 \times d}$, which has factorization $\tilde{T}=\sum_{i=1}^r A_i \otimes B_i \otimes \tilde{C_i}$, where $\tilde{C}_i=PC_i$. {To understand this projection, denote $T_{(n)}$ as the mode $n$ matricization of the tensor $T$, which is the flattening of the tensor $T$ along the $n$th mode by stacking the matrix slices together as columns of $T_{(n)}$. To project $T$, we project its mode 3 matricization $T_{(3)}\in\mathbb{R}^{m_1m_2 \times n}$ to obtain the projection of the mode 3 matricization $\tilde{T}_{(3)}\in\mathbb{R}^{m_1m_2 \times d}$ of $\tilde{T}$ by computing $\tilde{T}_{(3)}=T_{(3)}P^T$.}  We decompose $\tilde{T}$ in the projected space to obtain the factors $\tilde{A},\tilde{B},\tilde{C}$. Our estimates $\hat{A},\hat{B},\hat{C}$ for the original factors are $\hat{A}=\tilde{A}, \hat{B}=\tilde{B}$ and $\hat{C}$ is obtained by solving the compressive sensing problem in Eq. \ref{eq:basis-pursuit} for each column $C_i$. As above, this yields $r$ instances of Eq. \ref{eq:basis-pursuit}.
	 
%	 \emph{Linear classification.} For the problem of classifying data points $x^{(i)}\in \mathbb{R}^n$, $1\le i\le m$, we first perform a random projection to project the points into $d$ dimensions using the projection matrix $P$. Hence the projected points $\tilde{x}^{(i)}\in \mathbb{R}^d$ are given by $\tilde{x}^{(i)}=Px^{(i)}$. We then solve the classification problem in the projected space to learn a classifier $\tilde{w}^*$. Finally, we use compressive sensing to recover an estimate of the true classifier $\hat{w}^*$ from $\tilde{w}^*$.
%\end{enumerate}

\subsection{Choosing the projection matrix $P$}\label{sec:proj}

There are several desiderata which we require from our projection matrix $P$---

\begin{enumerate}
	\item  The first, more obvious, desiderata is that we should be able to solve the compressive sensing problem to recover the sparse solution in the original space from the solution in the projected space.
	\item For computational efficiency, we want projections which are efficient to compute, and which have the property that the sparse recovery problem can be solved efficiently using them.
	\item A more subtle requirement is that $P$ should be chosen such that if $w^*$ is the optimal solution in the original space, then the solution in the projected space is $\tilde{w}^*=Pw^*$, so that compressive sensing based recovery can then be carried out. This requires uniqueness of the optimization problem in the projected space, the requirement for which could depend on the original optimization problem. In Section \ref{sec:theory} we analyze these requirements for NMF and tensor decomposition.
\end{enumerate}

We now describe our choice of the projection matrix $P$. Consider a sparse projection matrix $P\in \{0,1\}^{d \times n}$ such that every column of $P$ has exactly $p$ non-zero entries, we refer to $p$ as the number of buckets, because each coordinate in the original $n$ dimensional space contributes to $p$ locations in the projected $d$ dimensional space. Let the support of the non-zero entries of each column of $P$ be chosen independently and uniformly at random. We will rely on seminal work on compressive sensing using sparse projection matrices for recovering the sparse solution efficiently from the projected solution. \cite{berinde2008combining,berinde2008practical,berinde2009sequential,indyk2008near}. We use the Sequential Sparse Matching Pursuit (SSMP) algorithm \cite{berinde2009sequential} for our recovery step instead of solving the LP. The SSMP algorithm allows linear time recovery of the original vector for sparse projection matrices, whereas the worst case time complexity of solving LPs can be cubic, and it also outperforms the LP formulation in practice \cite{berinde2009sequential}. 

\begin{thm}
	With high probability, a randomly chosen $P$ according to the above construction can be used for the recovery of $k$-sparse signals using either the linear programming formulation or the more efficient Sequential Sparse Matching Pursuit (SSMP) method.
\end{thm}
\begin{proof}
	The key property of $P$ which enables compressive sensing is that $P$ is the adjacency matrix of a \emph{bipartite expander} \cite{hoory2006expander}. Consider a bipartite graph $G$ with $n$ nodes on the left part and $d$ nodes on the right part such that every node in the left part has degree $p$. We call $G$ a $(\gamma n,\alpha)$ expander if every subset of at most $t\le \gamma n$ nodes in $U$ has at least $\alpha tp$ neighbors in $V$. It is not difficult to show that a randomly chosen matrix $P$ with $p$ non-zero entries per column is the adjacency matrix of a $(\gamma n, 4/5)$ expander for $\gamma n=d/(pe^5)$ with high probability if $p=O(\log n)$. We formally prove this as Lemma \ref{expander} in Appendix \ref{sec:expander}. 
	
	For the basis pursuit problem described in (\ref{eq:basis-pursuit}), seminal results in compressive sensing \cite{donoho2006compressed,candes2008restricted,candes2006near} show that using dense projection $P$ guarantees recovery with $d=O(k\log n)$ if the original solution is $k$-sparse. This property was subsequently extended to sparse projection matrices, and we will leverage this fact. Theorem 3 of \citet{berinde2008combining} shows that if $x$ is $k$-sparse, then with $P$ as defined above $x$ can be recovered from $Px$ using the LP if $P$ is the adjacency matrix of a $(2k,4/5)$ expander. A randomly chosen $P$ with $d=O(k\log n)$ will be a $(2k,4/5)$ expander with high probability (Lemma \ref{expander}), and hence can be used for sparse recovery of $k$-sparse signals.
\end{proof}

Note that as $P$ is sparse, the projection step can also be carried out efficiently.   Hence using $P$ defined as above satisfies our desiderata (1) and (2) for the projection matrix---that the sparse recovery step is computationally efficient and provably works if the original solution $w^*$ is $k$-sparse and the solution $\tilde{w}^*$ in the projected space is $\tilde{w}^*=Pw^*$.
  %We assume throughout the paper that the solution to the original optimization problem is $k$-sparse (for the problem of recovering matrices, we assume every factor in $\mathbb{R}^n$ is $k$-sparse).

However, we still need to ensure desiderata (3)---that the solution $\tilde{w}^*=Pw^*$. We analyze when this is the case for NMF and tensor decomposition next in Section \ref{sec:theory}. We summarize these conditions in Table \ref{tab:cond} for NMF and tensor decomposition. Note that the bounds suggested by our theoretical results are tight up to logarithmic factors, as projecting the matrix or the tensor to dimension below the rank will not preserve uniqueness of the decomposition.

\begin{table*}[]
	\centering
	\caption{Parameters for the projection matrix $P\in\{0,1\}^{d\times n}$ suggested by our theoretical analysis for NMF and tensor decomposition (TD). $p$ is the number of non-zero entries per column of $P$.}
	\label{tab:cond}
	\begin{tabular}{@{}cccc@{}}
		\toprule
	Task	& Parameter  & Number of buckets $p$ & Projection dimension $d$ \\ \midrule
	NMF	& $r$: rank of matrix  & $O(\log n)$  & $O((r+k)\log n)$ \\ \midrule
	TD	& $r$: rank of tensor & $O(\log n)$ & $\max\{r,O(k\log n)\}$
	\end{tabular}
\end{table*}

% \subsection{Solving the compressing sensing problem}

%\noindent \emph{Choosing the projection matrix $P$: }

%\noindent \emph{Solving the compressing sensing problem: }
